Class-Specific Explainability for Deep Time Series Classifiers

Explainability helps users trust deep learning solutions for time series classification. However, existing explainability methods for multi-class time series classifiers focus on one class at a time, ignoring relationships between the classes. Instead, when a classifier is choosing between many classes, an effective explanation must show what sets the chosen class apart from the rest. We now formalize this notion, studying the open problem of class-specific explainability for deep time series classifiers, a challenging and impactful problem setting. We design a novel explainability method, DEMUX, which learns saliency maps for explaining deep multi-class time series classifiers by adaptively ensuring that its explanation spotlights the regions in an input time series that a model uses specifically to its predicted class. DEMUX adopts a gradient-based approach composed of three interdependent modules that combine to generate consistent, class-specific saliency maps that remain faithful to the classifier's behavior yet are easily understood by end users. Our experimental study demonstrates that DEMUX outperforms nine state-of-the-art alternatives on five popular datasets when explaining two types of deep time series classifiers. Further, through a case study, we demonstrate that DEMUX's explanations indeed highlight what separates the predicted class from the others in the eyes of the classifier. Our code is publicly available at https://github.com/rameshdoddaiah/DEMUX.

==> algo_tspert.tex <==
%----------------------------------------------------------------
% Figure: Algorithm
% \usepackage{placeins}

\begin{figure*}[t]
% \begin{figure}[!htbp]
\center
\begin{tabular}{l}
\hline\vspace{-4pt}\\
  \textbf{Input:}\\
  \begin{tabular}{l@{: }l@{ }l@{: }l}
	$TS$ & Original Time Series Instance, &$L$ & Original Classification Label.\\
	$TV\_norm$ & Tv norm coefficient, & $Noise\_Amt$ & The Amount of Noise to Add.\\
	$Blur\_Amt$ & The Amount of Blur to Add, & $Budget$ & The Amount of budget coefficient.\\
	$MSE$ & The Amount of MSE coefficient, & $Max\_Itr$ & Maximum \# of iteration.\\
	$Class\_0\_Mean$ & Mean of all Class 0 labels , & $Class\_1\_Mean$ & Mean of all Class 1 labels.\\
  \end{tabular}\vspace{5pt}\\
\textbf{Training:}\\
%-----------------------------------------------
\quad - Initialize the gradient mask(Mask) to one.\\
\quad - Blur\_TS = Blur\_Amt of Gaussian and Median blur per time step.\\
\quad - Initialize Adam Optimizer for gradient mask.\\
\quad - For $epochs=1, \cdots, Max\_Itr$:\\
\quad\quad 1. Negative\_Mask = 1-Mask\\
\quad\quad 2. Zt = Pick a random Time Series from Test Data Set as replacement strategy\\
\quad\quad 3. Perturbed\_Input = TS*Mask + Zt*(1-Mask)\\
\quad\quad 4. Perturbed\_Input = Perturbed\_Input+Blur\_Ts*Mask\\
\quad\quad 5. Perturbed\_Input = Perturbed\_Input+Add Noise\_Amt of random noise for each Time Step\\
\quad\quad 6. New\_Classification\_Label(NL) = Get New Black\_Box\_Model Prediction with (Perturbed\_Input)\\
\quad\quad 7. MSE\_Loss\_Component = MSE * Mean squared error\ loss\ between(L,NL)\\
\quad\quad 8. Budget\_Loss\_Component = Budget * Mean(Mask)\\
\quad\quad 9. TV\_norm\_Loss\_Component = TV\_norm * TV norm of (Mask, TV\_Beta)\\

\quad\quad 10. Loss = MSE\_Loss\_Component + Budget\_Loss\_Component + TV\_norm\_Loss\_Component \\
\quad\quad 11. Back Propagate the Loss\\
\quad\quad 12. Take Optimizer Step \\
\quad\quad 13. Clamp Mask Gradients between 0 to 1 \\
\quad - Repeat until convergence or \#iteration$> Max\_It$\\
% \quad\quad 14. If early stop criteria is enabled and new output prediction percentage is lower than \\
\quad - Computed Gradient Mask is the Saliency Mask which is sent to Insertion and Deletion AUC algorithm\\

% \sout{
% %-----------------------------------------------
% \textbf{Insertion AUC:}\\
% \quad - Quick Sort the obtained Saliency Mask \\
% \quad\quad 1. if L is Class 0 then use Class\_1\_Mean as new Time Series \\
% \quad\quad 2. if L is Class 1 then use Class\_0\_Mean as new Time Series \\

% \quad - For $step =1, \cdots, Max\_Time\_Steps$:\\
% \quad\quad 1. Evaluate the model with new Time Series and get new Classification result \\
% \quad\quad 2. Replace top most saliency value's time step with opposite class's mean value in new Time Series\\
% \quad\quad 3. remove top most saliency value from the sorted list \\
% \quad\quad 4. Save new Classification result to Insertion AUC list\\
% \quad - Repeat until convergence or \#steps$> Max\_Time\_Steps$\\


% \textbf{Deletion AUC:}\\
% \quad - Quick Sort the obtained Saliency Mask \\
% \quad - For $step =1, \cdots, Max\_Time\_Steps$:\\
% \quad\quad 1. Evaluate the model with TS and get new Classification result \\
% \quad\quad 2. Replace top most saliency value's time step in TS with opposite class's mean value\\
% \quad\quad 3. Save new Classification result to Deletion AUC list\\
% \quad - Repeat until convergence or \#steps$> Max\_Time\_Steps$\\
% }
%-----------------------------------------------
  \hline
  \end{tabular}\vspace{5pt}
  \caption{The Neural Time Series algorithm}\label{fig:algorithm_nte}
\end{figure*}
%---------------------------------------------------------------------------


==> equations.tex <==
we are given a set of $N$ time series $\mathcal{D} = \{x_1, \dots,x_N\}$

$f:\mathbb{X} \to \mathcal{Y}$, where $\mathbb{X} \in \mathbb{R}^D$ is the $D$-dimensional feature space and $\mathcal{Y} = \{1,2,\dots,C\}$  is the label space with $C$ classes.

instance-of-interest $X \in \mathcal{D}$ where $X = [x_1, \dots, x_T]$

predicted probability distribution $\mathbf{\hat{y}} = f(X)$ where $\mathbf{\hat{y}} \in \mathcal{Y}$ and $z = \argmax \mathbf{\hat{y}}$ as the class-of-interest with highest predicted probability

==> fig_1_butterfly.tex <==
%-------------------------------------------------------
% Butterfly Figure
% The goal of this figure is to show case problem definition.
% In order to answer the reviewer's question on: what problem are you solving, why it is import/interesting
% Key points:
%   1) use simple and concrete example 
%   2) colorful 
%   3) should look interesting 
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example figure to fill the space before you finish your own figure
%-------------------------------------------------------
\begin{figure}[t]
\centering
    \begin{minipage}[l]{\columnwidth}
        \centering
  	    \includegraphics[width=\textwidth]{fig/butterfly.pdf}
    \end{minipage}
\caption{An Example of Dual Active Feature and Sample Selection Problem in Graph Data.}
\label{fig:dual_example}

% squeeze some vertical space between caption and main text (Note: some conferences may not allow this)
\vspace{-10pt}

\end{figure}
%-------------------------------------------------------


==> fig_2_family.tex <==
%-------------------------------------------------------
% Family Portrait Figure (show novelty)
% The goal of this figure is to show the similarity and difference between our work with related works.
% In order to answer the reviewer's question on: what is the novelty of the paper?
% Key points:
%   1) Show both similarities and difference. 
%      The similarities are to prove that we are comparing with closely related work. So we know the state-of-the-art.
%      The differencies are to show the key contributions of our model or our new problem or framework.
%   2) If we want to claim the novelty in new problem definition, compare with related problems.
%   3) If we want to claim the novelty in new models, compare with related method on framework/highlevel design.
%   4) Don't use toy data here. Use toy data in Jenny-Craig figure. 
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example figure to fill the space before you finish your own figure
%-------------------------------------------------------
\begin{figure}[t]
\centering
\subfigure[Collective Classification]{
   \label{fig:comp_slcc}
   \begin{minipage}[c]{\columnwidth}
        \centering
		\includegraphics[width=.8\textwidth]{fig/family1.pdf}
   \end{minipage}
}

\subfigure[Multi-Label Classification]{
   \label{fig:comp_ml}
   \begin{minipage}[c]{\columnwidth}
        \centering
		\includegraphics[width=.8\textwidth]{fig/family2.pdf}
   \end{minipage}
}

\subfigure[Multi-Label Collective Classification]{
    \label{fig:comp_mlcc}
    \begin{minipage}[l]{\columnwidth}
      \centering
  	\includegraphics[width=.8\textwidth]{fig/family3.pdf}
    \end{minipage}
}

% squeeze some vertical space between image and caption (Note: some conferences may not allow this)
\vspace{-10pt}

\caption{
    Comparison of the settings for different classification problems. 
    Each rectangle represents an instance. 
    $\mathbf{X}_i$ denotes the attributes of the instance, and $Y_i$ or $Y_i^k$ denotes a class label. 
    Instances directly linked by an edge are related.
}
\label{fig:comp_prob}

% squeeze some vertical space between caption and main text (Note: some conferences may not allow this)
\vspace{-10pt}

\end{figure}
%-------------------------------------------------------




==> fig_3_jenny.tex <==
%-------------------------------------------------------
%  Jenny Craig Figure
% The goal of this figure is to show how your method works in a toy dataset.
% Key points:
%   1) Show a toy dataset, as simple as possible.
%   2) Before:Show the results of other methods 
%   3) After: Show the results of our methods 
%   4) Make sure the difference between BEFORE and AFTER is big 
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example figure to fill the space before you finish your own figure
%-------------------------------------------------------

%-------------------------------------------------------
\begin{figure*}
  \subfigure[A multi-label classification problem with three labeled instances]{\label{subfig:data}
    \begin{minipage}[r]{.65\columnwidth}
      \centering
      \includegraphics[width=0.78\textwidth]{fig/jenny1}\vspace{3pt}
    \end{minipage}

  }
  \subfigure[ An approach by combining supervised single-label classification results]{\label{subfig:slsup}
    \begin{minipage}[r]{.65\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/jenny2}\vspace{3pt}
    \end{minipage}
  }
  \subfigure[An approach by supervised multi-label classification]{\label{subfig:mlsup}
    \begin{minipage}[r]{.65\columnwidth}
      \centering
      \includegraphics[width=.98\textwidth]{fig/jenny3}\vspace{3pt}
    \end{minipage}
  }
  \subfigure[An approach by adopting single-label transductive classification results]{\label{subfig:sllp}
    \begin{minipage}[r]{.65\columnwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{fig/jenny4}\vspace{3pt}
    \end{minipage}
  }
  \subfigure[ Our approach: transductive multi-label classification]{\label{subfig:tram}
    \begin{minipage}[r]{.65\columnwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{fig/jenny5}\vspace{3pt}
    \end{minipage}
  }
  \caption{Different approaches on transductive multi-label classification problem. }
  \label{fig:example}
\end{figure*}
%-------------------------------------------------------




==> fig_4_algorithm.tex <==
%----------------------------------------------------------------
% Figure: Algorithm
% \usepackage{placeins}

\begin{figure*}[t]
% \begin{figure}[!htbp]
\center
\begin{tabular}{l}
\hline\vspace{-4pt}\\
  \textbf{Input:}\\
  \begin{tabular}{l@{: }l@{ }l@{: }l}
	$TS$ & Original Time Series Instance, &$L$ & Original Classification Label.\\
	$TV\_norm$ & Tv norm coefficient, & $Noise\_Amt$ & The Amount of Noise to Add.\\
	$Blur\_Amt$ & The Amount of Blur to Add, & $Budget$ & The Amount of budget coefficient.\\
	$MSE$ & The Amount of MSE coefficient, & $Max\_Itr$ & Maximum \# of iteration.\\
	$Class\_0\_Mean$ & Mean of all Class 0 labels , & $Class\_1\_Mean$ & Mean of all Class 1 labels.\\
  \end{tabular}\vspace{5pt}\\
\textbf{Training:}\\
%-----------------------------------------------
\quad - Initialize the gradient mask(Mask) to one.\\
\quad - Blur\_TS = Blur\_Amt of Gaussian and Median blur per time step.\\
\quad - Initialize Adam Optimizer for gradient mask.\\
\quad - For $epochs=1, \cdots, Max\_Itr$:\\
\quad\quad 1. Negative\_Mask = 1-Mask\\
\quad\quad 2. Zt = Pick a random Time Series from Test Data Set as replacement strategy\\
\quad\quad 3. Perturbed\_Input = TS*Mask + Zt*(1-Mask)\\
\quad\quad 4. Perturbed\_Input = Perturbed\_Input+Blur\_Ts*Mask\\
\quad\quad 5. Perturbed\_Input = Perturbed\_Input+Add Noise\_Amt of random noise for each Time Step\\
\quad\quad 6. New\_Classification\_Label(NL) = Get New Black\_Box\_Model Prediction with (Perturbed\_Input)\\
\quad\quad 7. MSE\_Loss\_Component = MSE * Mean squared error\ loss\ between(L,NL)\\
\quad\quad 8. Budget\_Loss\_Component = Budget * Mean(Mask)\\
\quad\quad 9. TV\_norm\_Loss\_Component = TV\_norm * TV norm of (Mask, TV\_Beta)\\

\quad\quad 10. Loss = MSE\_Loss\_Component + Budget\_Loss\_Component + TV\_norm\_Loss\_Component \\
\quad\quad 11. Back Propagate the Loss\\
\quad\quad 12. Take Optimizer Step \\
\quad\quad 13. Clamp Mask Gradients between 0 to 1 \\
\quad - Repeat until convergence or \#iteration$> Max\_It$\\
% \quad\quad 14. If early stop criteria is enabled and new output prediction percentage is lower than \\
\quad - Computed Gradient Mask is the Saliency Mask which is sent to Insertion and Deletion AUC algorithm\\

% \sout{
% %-----------------------------------------------
% \textbf{Insertion AUC:}\\
% \quad - Quick Sort the obtained Saliency Mask \\
% \quad\quad 1. if L is Class 0 then use Class\_1\_Mean as new Time Series \\
% \quad\quad 2. if L is Class 1 then use Class\_0\_Mean as new Time Series \\

% \quad - For $step =1, \cdots, Max\_Time\_Steps$:\\
% \quad\quad 1. Evaluate the model with new Time Series and get new Classification result \\
% \quad\quad 2. Replace top most saliency value's time step with opposite class's mean value in new Time Series\\
% \quad\quad 3. remove top most saliency value from the sorted list \\
% \quad\quad 4. Save new Classification result to Insertion AUC list\\
% \quad - Repeat until convergence or \#steps$> Max\_Time\_Steps$\\


% \textbf{Deletion AUC:}\\
% \quad - Quick Sort the obtained Saliency Mask \\
% \quad - For $step =1, \cdots, Max\_Time\_Steps$:\\
% \quad\quad 1. Evaluate the model with TS and get new Classification result \\
% \quad\quad 2. Replace top most saliency value's time step in TS with opposite class's mean value\\
% \quad\quad 3. Save new Classification result to Deletion AUC list\\
% \quad - Repeat until convergence or \#steps$> Max\_Time\_Steps$\\
% }
%-----------------------------------------------
  \hline
  \end{tabular}\vspace{5pt}
  \caption{The Neural Time Series algorithm}\label{fig:algorithm_nte}
\end{figure*}
%---------------------------------------------------------------------------


==> sec_2_problem_def.tex <==



\section{Problem Formulation} 
\label{sec:problem}
Assume we are given a set of $N$ time series $\mathcal{D} = \{X^1, \dots, X^N\}$ and a classifier $f:\mathbb{X} \to \mathcal{Y}$, where $\mathbb{X} \in \mathbb{R}^T$ is the $T$-dimensional feature space and $\mathcal{Y}$ is the label space.
Let us consider an instance-of-interest $\hat{X} \in \mathcal{D}$ where $\hat{X} = [\hat{x}_1, \dots, \hat{x}_T]$ along with a class-of-interest $C$, the prediction for which we would like an explanation.
Our goal is to derive a \snote{saliency} vector (\snote{changing $r_{t}$ to $s_{t}$ as $r_{t}$ is used to convey replacement time-series. }) $s = [s_1, \dots, s_T ]$ where $s_t \in [-1, 1]$ indicates the \textit{importance} of time step $t$ with respect to $P(C|\hat{X})$, the probability of class $C$ as predicted by $f$.
The scale of the real-valued $s_t$ reflects the importance of the corresponding $x_t$.

While the notion of \textit{importance} is challenging to quantify, we follow the lead of recent work on perturbation-based explainability \snote{\cite{Fong2017InterpretableEO, fong2019understanding}} and assume that it is a reflection of the \textit{expected scale of the change in $P(C|\hat{X})$ when $\hat{X}$ is perturbed}: $|P(C|\hat{X}) - P(C|\hat{X}^\prime)|$, where $\hat{X}^\prime$ is a perturbed version of $\hat{X}$.
Naturally, the perturbation-based explanation problem is thus to derive a perturbation function $\phi(\hat{X})$ that can be used to discover the impact of perturbing each time step $\hat{x}_t$ on $P(C|\hat{X})$ under the intuition that the more a time step can be changed without impacting $P(C|\hat{X})$, the less important the time step.
A successful importance vector $s$ will assign high values to the most-impactful time steps, effectively ranking them by their impact on $P(C|\hat{X})$.
Intuitively, an explanation that is \textit{simpler} is often easier to understand, and so we also prefer that $\sum_{t=1}^{T}s_t$ be small to highlight only the most-important time steps.



==> tab_1_notation.tex <==
%-------------------------------------------------------
% Table of Math Notations 
% The goal is to have a map of the notation system, so that reviewers can easily find the meaning of each notation.
% Use different fonts/formats for different kinds of notations.
% Guidelines:
%   set: e.g. {1,2,3}, use upper case: \mathcal{X}
%   vector: e.g. (1,2,3), use bolded lower case: \mathbf{x}
%   scalar random variable: e.g. X \in\{0,1\}, use upper case: X
%   scalar constant: e.g. x = 1, use lower case: x
%   Space: infinite set, e.g., a \in R, use upper case: \mathbb{R}
%   Matix: e.g., [[0,1],[2,3]], use bolded upper case: \mathbf{X}
%  For more details: see http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


%----------------------------------------------------------------
% Tabel 1: notations
\begin{table*}[t]
    \centering 
    \caption{Important Notations.}\vspace{10pt}\label{tab:notation}
    \begin{tabular}{|r|l|}
    \hline\vspace{-8pt}&\\
    Symbol& Definition\\
    \hline\vspace{-8pt}&\\
    $\mathcal{V}=\{v_1, \cdots, v_n\}$ & the set of nodes\\
    $\mathcal{E}=\{e_i\in \mathcal{V}\times\mathcal{V}\}$  &the set of edges or links\\
    $\mathcal{N}(i)$ or  $\mathcal{N}(v_i, \mathcal{E})$   & the index set of all nodes directly-linked to $v_i$ with edges in $\mathcal{E}$\\
    $\mathcal{X}=\{\mathbf{x}_1, \cdots, \mathbf{x}_n\}$ & the given attribute values for each node\\
    $\mathcal{Y}= \left\{\mathbf{Y}_1, \cdots, \mathbf{Y}_n\right\}$   &the set of variables for label sets of the nodes\\
    $\mathbf{Y}_i=\left(Y_i^1, \cdots, Y_i^q\right)$ & the vector of variables for the label set of node $v_i$, and $Y_i^k\in\{0,1\}$\\
    $L$ and $U$ & the index sets for training nodes and testing nodes, and $L\cup U = \{1, \cdots, n\}$\\
    $\mathbf{y}_i =\left(y_i^1, \cdots, y_i^q\right)$      &  the given label sets for node $v_i$ ($i\in L$), and $Y_i^k =y_i^k$\\
    \vspace{-8pt}&\\\hline\vspace{-8pt}&\\
    $\mathbf{Y}^k=\left(Y_1^k, \cdots, Y_n^k\right)$ & the vector of variables for the $k$-th label\\
    $\mathbf{Y}^{-k}_i =\left(\cdots, Y_i^{k-1}, Y_i^{k+1}, \cdots\right)$  &  the vector of all the $Y_i^p$ variables with indices $\{p | p\ne k\}$ \\
    $\mathbf{y}^{-k}_i =\left( \cdots, y_i^{k-1}, y_i^{k+1}, \cdots\right)$  &  the vector of all the $y_i^p$ values with indices $\{p | p\ne k\}$ \\
    $\mathbf{Y}^{-k}_{j\in \mathcal{N}(i)}$  &  the vector of all the $Y_j^p$ variables with indices $\{(p,j) | p\ne k, j \in \mathcal{N}(i)\}$ \vspace{2pt}\\
    
     \hline
    \end{tabular}
\end{table*}
%---------------------------------------------------------------------------


==> tab_2_dataset.tex <==
%-------------------------------------------------------
% Table of Datasets 
% The goal is to summarize the statistics about the dataset to show the reviewers that the datasets are reasonable.
% Key points:
%   1) include 3 or more datasets (1 or 2 datasets will look weak, will be very likely to be questioned by reviewers)
%   2) make sure the datasets are/look large. e.g., more than 2000 sample/nodes/connections ...
%   3) make sure that most of the datasets are real-world datasets. Not synthetic datasets.
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------

%%----------------------------------------------------------------
%% Table : Dataset Statistics
\begin{table}[t]
    \centering
    \caption{Summary of experimental datasets. ``Ave. Card'' denotes the average cardinality of label sets assigned to the nodes.}\vspace{10pt}\label{tab:datastat}
    \begin{tabular}{lrrr}
        \hline\vspace{-8pt}\\
            & \multicolumn{3}{c}{Data Sets}\\
            \cline{2-4}\vspace{-8pt}\\
            Characteristics
            & DBLP-A
            & DBLP-B
            & IMDB\vspace{2pt}\\
        \hline\vspace{-8pt}\\
        \# Feature	&687 &699   &586 \\
        \# Nodes  	&4638 &4559  &4081\\
        \# Links    &16447 &14407  &41087\\
         \# Class 	&6	&6 &22\\
         Ave. Card	&1.70 &1.24 &2.13\vspace{2pt}\\
        \hline
    \end{tabular}
    \label{table:Dataset}
\end{table}
%----------------------------------------------------------------


==> tab_3_baseline.tex <==
%-------------------------------------------------------
% Table of Baselines 
% The goal is to summarize the compared methods to show the reviewers that the baselines are reasonable.
% Key points:
%   1) include 5 or more baselines including our method (only comparing with 2 baselines will look weak, will be very likely to be questioned by reviewers)
%   2) make sure some of the baselines are recent works and related (state-of-the-art). e.g., add citations to them
%   3) make sure by comparing the pairs of baselines we can support the major claims of the paper. For example, if our method is designed with feature A+B, we need to compare with (A only) and (B only) baselines. If (A+B) is better than (A only), the result support the claim that B is important and crucial. If (A+B) is also better than (B only), the result support the claim that A is important and crucial. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------

%----------------------------------------------------------------
% Tabel 3: Baseline methods being compared 
\begin{table*}[t]
    \centering
    \caption{Summary of compared methods.}\vspace{10pt}\label{tab:method}
    \begin{tabular}{|l|c|l|c|}
    \hline&&&\vspace{-8pt}\\
                & \textbf{Type of} 
                & \multicolumn{1}{c|}{\textbf{Dependencies}}
                & \\
        \textbf{Method}
        &  \textbf{Classification}
        & \multicolumn{1}{c|}{\textbf{Exploited}}
        & \textbf{Publication}\\
    \hline\hline \vspace{-10pt}&&&\\
    BSVM & Binary Classification & \multicolumn{1}{c|}{All Independent} &\cite{BLSB04}\\ \hline\vspace{-10pt}&&&\\
    CC    & Multi-Label Classification&\ding{172} Intra-Instance Cross-Label Dependency& \cite{RPHF09}\\ \hline\vspace{-10pt}&&&\\
    ECC   & Multi-Label Classification&\ding{172} Intra-Instance Cross-Label Dependency& \cite{RPHF09}\\ \hline\vspace{-10pt}&&&\\
    SL-ICA & Collective Classification &\ding{173} Inter-Instance Single-Label Dependency& \cite{LG03}\\ \hline\vspace{-10pt}&&&\\
    ML-ICA & Multi-Label Collective Classification&\ding{173} Inter-Instance Single-Label Dependency & This paper\\       &&\ding{174} Inter-Instance Cross-Label Dependency &\\ \hline\vspace{-10pt}&&&\\
      		 &&\ding{172} Intra-Instance Cross-Label Dependency &\\
    ICML & Multi-Label Collective Classification&\ding{173} Inter-Instance Single-Label Dependency& This paper\\
             &&\ding{174} Inter-Instance Cross-Label Dependency &\\
    \hline
    \end{tabular}
\end{table*}
%---------------------------------------------------------------------------


==> tab_4_result.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[t]
\caption{Results on the ADNI (Alzheimer's Disease) dataset with different number of features($t=100, \cdots, 500$). The results are reported as ``average performance + (rank)". }\label{tab:adni}
{\tiny
\centering
\begin{tabular}{rlllllrlllllr}
\toprule
 & \multicolumn{5}{c}{Error Rate $\downarrow$}&&\multicolumn{5}{c}{F1 $\uparrow$}&Avg.\\
\cmidrule{2-6}\cmidrule{8-12}
{Methods}&\multicolumn{1}{c}{$t=100$}&\multicolumn{1}{c}{$t=200$}&\multicolumn{1}{c}{$t=300$}&\multicolumn{1}{c}{$t=400$}&\multicolumn{1}{c}{$t=500$}&&\multicolumn{1}{c}{$t=100$}&\multicolumn{1}{c}{$t=200$}&\multicolumn{1}{c}{$t=300$}&\multicolumn{1}{c}{$t=400$}&\multicolumn{1}{c}{$t=500$}&\multicolumn{1}{c}{Rank}\\
\midrule
{\color{red} Exp}-HSIC 				&0.400 {\color{blue} (9)} 		&	0.367 {\color{blue} (8)} 	&0.367 {\color{blue} (10)}&0.317 {\color{blue} (4)} 		&0.333 {\color{blue} (9)} 		&&0.699 {\color{blue} (9)} 	&0.725 {\color{blue} (9)} 		&0.725 {\color{blue} (9)} 	&0.753 {\color{blue} (6)} 		&0.743 {\color{blue} (10)} 		&{\color{blue} (8.3)}\\
{\color{green} Med}-HSIC  				&0.433 {\color{blue} (14)} 	&	0.350 {\color{blue} (5)} 	&0.333 {\color{blue} (6)} 	&0.350 {\color{blue} (8)} 		&0.317 {\color{blue} 
6
 (7)} 		&&0.667 {\color{blue} (13)} 	&0.741 {\color{blue} (7)} 		&0.757 {\color{blue} (4)} 	&0.734 {\color{blue} (9)} 		&0.766 {\color{blue} (7)} 		&{\color{blue} (8.0)}\\
{\color{violet} Mod}-HSIC 				&0.367 {\color{blue} (6)} 		&	0.333 {\color{blue} (3)} 	&0.300 {\color{blue} (1)*} 	&0.317 {\color{blue} (4)} 		&0.300 {\color{blue} (2)} 		&&0.703 {\color{blue} (8)} 	&0.750 {\color{blue} (4)} 		&0.776 {\color{blue} (3)} 	&0.766 {\color{blue} (3)} 		&0.775 {\color{blue} (4)} 		&{\color{blue} (3.8)}\\
{\color{blue} $\varphi$Pr}-HSIC	&0.283 {\color{blue} (1)*}	&	0.283 {\color{blue} (1)*} 	&0.333 {\color{blue} (6)} 	&0.333 {\color{blue} (7)} 		&0.300 {\color{blue} (2)} 		&&0.778 {\color{blue} (1)*}	&0.785 {\color{blue} (1)*}	&0.757 {\color{blue} (4)} 	&0.750 {\color{blue} (7)} 	&0.776 {\color{blue} (3)} 		&{\color{blue} (3.3)}\\
{\it \color{gray} HSIC}	&0.450 {\color{blue} (16)}	&		0.467 {\color{blue} (19)} 	&	0.467 {\color{blue} (17)} 	&	0.500 {\color{blue} (18)} 		&	0.500 {\color{blue} (18)} 		&&0.615 {\color{blue} (18)}	&	0.597 {\color{blue} (19)}	&	0.622 {\color{blue} (17)} 	&	0.583 {\color{blue} (18)} 	&0.584 {\color{blue} (18)} 		&{\color{blue} (18.1)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Ratio 				&0.433 {\color{blue} (14)} 	&	0.383 {\color{blue} (10)} 	&0.317 {\color{blue} (4)} 	&0.300 {\color{blue} (2)} 		&0.300 {\color{blue} (2)} 		&&0.667 {\color{blue} (13)} 	&0.715 {\color{blue} (10)}	&0.756 {\color{blue} (6)} 	&0.766 {\color{blue} (3)} 		&0.766 {\color{blue} (7)} 		&{\color{blue} (7.1)}\\
{\color{green} Med}-Ratio 				&0.450 {\color{blue} (16)} 	&	0.417 {\color{blue} (15)} 	&0.450 {\color{blue} (16)}&0.383 {\color{blue} (11)} 	&0.383 {\color{blue} (11)} 		&&0.639 {\color{blue} (17)} 	&0.653 {\color{blue} (16)}	&0.608 {\color{blue} (20)} &0.689 {\color{blue} (12)} 	&0.684 {\color{blue} (11)} 		&{\color{blue} (14.5)}\\
{\color{violet} Mod}-Ratio 				&0.317 {\color{blue} (3)} 		&	0.350 {\color{blue} (5)} 	&0.433 {\color{blue} (15)}&0.417 {\color{blue} (13)} 	&0.467 {\color{blue} (15)} 		&&0.776 {\color{blue} (2)} 	&0.744 {\color{blue} (6)} 		&0.659 {\color{blue} (13)}&0.657 {\color{blue} (13)} 	&0.612 {\color{blue} (15)} 		&{\color{blue} (9.9)}\\
{\color{blue} $\varphi$Pr}-Ratio	&0.400 {\color{blue} (9)} 		&	0.317 {\color{blue} (2)} 	&0.300 {\color{blue} (1)*} 	&0.300 {\color{blue} (2)} 		&0.267 {\color{blue} (1)*} 		&&0.692 {\color{blue} (10)} 	&0.764 {\color{blue} (2)} 		&0.784 {\color{blue} (1)*} 	&0.778 {\color{blue} (2)} 	&0.809 {\color{blue} (1)*} 		&{\color{blue} (3.1)}\\
{\it \color{gray} Ratio} 				&0.500 {\color{blue} (19)} 	&		0.483 {\color{blue} (20)} 	&	0.533 {\color{blue} (22)} 	&	0.567 {\color{blue} (22)} 		&	0.533 {\color{blue} (20)} 		&&0.581 {\color{blue} (20)} 	&	0.603 {\color{blue} (18)}	&	0.533 {\color{blue} (21)} 	&	0.519 {\color{blue} (22)} 		&	0.550 {\color{blue} (20)} 		&{\color{blue} (20.4)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Gtest 				&0.300 {\color{blue} (2)} 		&	0.367 {\color{blue} (8)} 	&0.317 {\color{blue} (4)} 	&0.350 {\color{blue} (8)} 		&0.383 {\color{blue} (11)} 		&&0.774 {\color{blue} (3)} 	&0.693 {\color{blue} (11)}	&0.729 {\color{blue} (9)} 	&0.702 {\color{blue} (10)} 	&0.672 {\color{blue} (12)} 		&{\color{blue} (7.8)}\\
{\color{green} Med}-Gtest 				&0.517 {\color{blue} (21)} 	&	0.450 {\color{blue} (18)} 	&0.400 {\color{blue} (11)}&0.500 {\color{blue} (18)} 	&0.483 {\color{blue} (17)} 		&&0.562 {\color{blue} (21)} 	&0.597 {\color{blue} (19)}	&0.655 {\color{blue} (14)}&0.567 {\color{blue} (19)} 	&0.589 {\color{blue} (17)} 		&{\color{blue} (17.5)}\\
{\color{violet} Mod}-Gtest 				&0.517 {\color{blue} (21)} 	&	0.550 {\color{blue} (22)} 	&0.500 {\color{blue} (21)}&0.500 {\color{blue} (18)} 	&0.517 {\color{blue} (19)} 		&&0.531 {\color{blue} (22)} 	&0.491 {\color{blue} (22)}	&0.527 {\color{blue} (22)}&0.545 {\color{blue} (20)} 	&0.558 {\color{blue} (19)} 		&{\color{blue} (20.6)}\\
$\varphi$Pr-Gtest	&0.450 {\color{blue} (16)} 	&	0.417 {\color{blue} (15)} 	&0.417 {\color{blue} (13)}&0.383 {\color{blue} (11)} 	&0.300 {\color{blue} (2)} 		&&0.648 {\color{blue} (16)} 	&0.675 {\color{blue} (14)}	&0.665 {\color{blue} (12)}&0.701 {\color{blue} (11)} &0.768 {\color{blue} (6)} 		&{\color{blue} (11.6)}\\
{\it \color{gray} Gtest} 				&0.500 {\color{blue} (19)} 		&		0.500 {\color{blue} (21)} 	&	0.467 {\color{blue} (17)} 	&	0.433 {\color{blue} (14)} 		&	0.550 {\color{blue} (21)}  &&0.583 {\color{blue} (19)} 	&	0.580 {\color{blue} (21)}	&	0.612 {\color{blue} (19)} 	&	0.656 {\color{blue} (14)} 	&	0.547 {\color{blue} (21)} 		&{\color{blue} (18.6)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Conf 				&0.367 {\color{blue} (7)} 		&	0.333 {\color{blue} (3)} 	&0.300 {\color{blue} (1)*} 	&0.283 {\color{blue} (1)*} 		&0.300 {\color{blue} (2)} 		&&0.744 {\color{blue} (6)} 	&0.762 {\color{blue} (3)} 		&0.780 {\color{blue} (2)} 	&0.795 {\color{blue} (1)*} 		&0.780 {\color{blue} (2)} 		&{\color{blue} *(2.8)}\\
{\color{green} Med}-Conf 				&0.333 {\color{blue} (4)} 		&	0.350 {\color{blue} (5)} 	&0.350 {\color{blue} (8)} 	&0.350 {\color{blue} (8)} 		&0.317 {\color{blue} (7)} 		&&0.760 {\color{blue} (4)} 	&0.747 {\color{blue} (5)} 		&0.752 {\color{blue} (7)} 	&0.740 {\color{blue} (8)} 		&0.770 {\color{blue} (5)} 		&{\color{blue} (6.1)}\\
{\color{violet} Mod}-Conf 				&0.417 {\color{blue} (12)} 	&	0.383 {\color{blue} (10)} 	&0.350 {\color{blue} (8)} 	&0.317 {\color{blue} (4)} 		&0.333 {\color{blue} (9)} 		&&0.690 {\color{blue} (11)} 	&0.728 {\color{blue} (8)} 		&0.742 {\color{blue} (8)} 	&0.759 {\color{blue} (5)} 		&0.750 {\color{blue} (9)} 		&{\color{blue} (8.4)}\\
{\color{blue} $\varphi$Pr}-Conf   &0.400 {\color{blue} (9)} 		&	0.417 {\color{blue} (15)} 	&0.467 {\color{blue} (17)}&0.467 {\color{blue} (16)} 	&0.433 {\color{blue} (13)} 		&&0.685 {\color{blue} (12)} 	&0.648 {\color{blue} (17)}	&0.619 {\color{blue} (18)}&0.592 {\color{blue} (17)} &0.632 {\color{blue} (13)} 		&{\color{blue} (14.7)}\\
{\it \color{gray} Conf}	&0.400 {\color{blue} (9)} 		&		0.400 {\color{blue} (13)} 	&	0.417 {\color{blue} (13)} 	&	0.450 {\color{blue} (15)} 		&	0.467 {\color{blue} (15)} 		&&0.655 {\color{blue} (15)} 	&	0.667 {\color{blue} (15)} 		&	0.645 {\color{blue} (15)} 	&	0.618 {\color{blue} (15)} 		&	0.610 {\color{blue} (16)} 		&{\color{blue} (14.1)}\\
\cmidrule{2-6}\cmidrule{8-12}
Exp-Freq	&0.383 {\color{blue} (8)} 		&	0.383 {\color{blue} (10)} 	&0.400 {\color{blue} (11)}&0.467 {\color{blue} (16)} 	&0.433 {\color{blue} (13)} 		&&0.705 {\color{blue} (7)} 	&0.685 {\color{blue} (13)}&0.675 {\color{blue} (11)} 	&0.607 {\color{blue} (16)} 	&0.632 {\color{blue} (13)} 		&{\color{blue} (11.8)}\\
{\it \color{gray} Freq }				&0.350 {\color{blue} (5)} 		&		0.400 {\color{blue} (13)} 	&	0.483 {\color{blue} (20)}&	0.550 {\color{blue} (21)} 	&	0.550 {\color{blue} (21)} 		&&0.747 {\color{blue} (5)} 	&	0.692 {\color{blue} (12)}&	0.627 {\color{blue} (16)} 	&	0.539 {\color{blue} (21)} 	&	0.547 {\color{blue} (21)} 		&{\color{blue} (15.5)}\\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Results on the ADHD (Attention Deficit Hyperactivity Disorder) dataset with different number of features ($t=100, \cdots, 500$). The results are reported as ``average performance + (rank)". }\label{tab:adhd}
{\tiny
\centering
\begin{tabular}{rlllllrlllllr}
\toprule
 & \multicolumn{5}{c}{Error Rate $\downarrow$}&&\multicolumn{5}{c}{F1 $\uparrow$}&Avg.\\
\cmidrule{2-6}\cmidrule{8-12}
{Methods}&\multicolumn{1}{c}{$t=100$}&\multicolumn{1}{c}{$t=200$}&\multicolumn{1}{c}{$t=300$}&\multicolumn{1}{c}{$t=400$}&\multicolumn{1}{c}{$t=500$}&&\multicolumn{1}{c}{$t=100$}&\multicolumn{1}{c}{$t=200$}&\multicolumn{1}{c}{$t=300$}&\multicolumn{1}{c}{$t=400$}&\multicolumn{1}{c}{$t=500$}&\multicolumn{1}{c}{Rank}\\
\midrule
{\color{red} Exp}-HSIC 				&0.423 {\color{blue} (10)}	&0.438 {\color{blue} (13)} 	&0.455 {\color{blue} (14)} 	&0.455 {\color{blue} (11)} 	&	0.448{\color{blue} (12)} 		&&0.593 {\color{blue} (10)} &	0.564 {\color{blue} (13)}	&0.543 {\color{blue} (14)} 	&0.547 {\color{blue} (11)}	&	0.549 {\color{blue} (12)}	&{\color{blue} (12.0)}\\
{\color{green} Med}-HSIC  				&0.420 {\color{blue} (9)} 		&0.405 {\color{blue} (8)} 		&0.413 {\color{blue} (8)} 		&0.448 {\color{blue} (10)} 	&	0.433 {\color{blue} (6)} 		&&0.569 {\color{blue} (13)} &	0.597 {\color{blue} (7)} 	&0.593 {\color{blue} (5)} 		&0.549 {\color{blue} (10)}	&	0.562 {\color{blue} (7)}		&{\color{blue} (8.3)}\\
{\color{violet} Mod}-HSIC 				&0.390 {\color{blue} (4)} 		&0.405 {\color{blue} (8)} 		&	0.403 {\color{blue} (4)} 	&0.393 {\color{blue} (1)*}	&0.410 {\color{blue} (2)} 			&&0.614 {\color{blue} (3)} 	&	0.599 {\color{blue} (6)} 	&0.596 {\color{blue} (4)} 		&0.594 {\color{blue} (1)*}	&0.584 {\color{blue} (2)}		&{\color{blue} *(3.5)}\\
{\color{blue} $\varphi$Pr}-HSIC	&0.432 {\color{blue} (12)} 	&0.470 {\color{blue} (17)} 	&0.475 {\color{blue} (16)} 	&0.513 {\color{blue} (22)} 	&	0.503 {\color{blue} (21)} 		&&0.597 {\color{blue} (7)} 	&	0.563 {\color{blue} (14)}	&0.554 {\color{blue} (13)} 	&0.508 {\color{blue} (17)}	&	0.525 {\color{blue} (18)}	&{\color{blue} (15.7)}\\
{\it \color{gray} HSIC}	&0.529 {\color{blue} (22)}	&	0.510 {\color{blue} (20)} 	&		0.488 {\color{blue} (17)} 	&	0.455 {\color{blue} (11)} 		&	0.485 {\color{blue} (17)} 		&&	0.505 {\color{blue} (22)}	&	0.494{\color{blue} (18)}	& 0.498 {\color{blue} (18)} 	&	0.538   {\color{blue} (13)} 	&0.526 {\color{blue} (17)} 		&{\color{blue} (17.5)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Ratio 				&0.388 {\color{blue} (3)} 		&0.400 {\color{blue} (5)} 		&0.415 {\color{blue} (10)} 	&0.440 {\color{blue} (8)} 		&	0.420 {\color{blue} (4)} 		&&0.613 {\color{blue} (4)} 	&	0.604 {\color{blue} (5)} 	&0.587 {\color{blue} (9)} 		&0.556 {\color{blue} (8)}		&0.576 {\color{blue} (4)}		&{\color{blue} (6.0)}\\
{\color{green} Med}-Ratio 				&0.450 {\color{blue} (16)} 	&0.418 {\color{blue} (11)} 	&0.388 {\color{blue} (1)*}	&0.428 {\color{blue} (6)} 		&	0.410 {\color{blue} (2)} 		&&0.554 {\color{blue} (15)} &	0.586 {\color{blue} (12)}	&0.619 {\color{blue} (1)*}	&0.571 {\color{blue} (5)}		&0.579 {\color{blue} (3)}		&{\color{blue} (7.2)}\\
{\color{violet} Mod}-Ratio 				&0.400 {\color{blue} (7)} 		&0.370 {\color{blue} (1)*}	&0.408 {\color{blue} (5)} 		&0.435 {\color{blue} (7)} 		&	0.428 {\color{blue} (5)} 		&&0.595 {\color{blue} (8)} 	&	0.634 {\color{blue} (1)*}	&0.591 {\color{blue} (7)} 		&0.558 {\color{blue} (7)}		&0.560 {\color{blue} (9)}		&{\color{blue} (5.7)}\\
{\color{blue} $\varphi$Pr}-Ratio	&0.372 {\color{blue} (1)*}	&0.430 {\color{blue} (12)} 	&0.410 {\color{blue} (7)} 		&0.415 {\color{blue} (2)} 		&	0.408 {\color{blue} (1)*} 		&&0.630 {\color{blue} (1)*} &	0.589 {\color{blue} (9)} 	&0.590 {\color{blue} (8)} 		&0.591 {\color{blue} (2)}		&0.589 {\color{blue} (1)*}	&{\color{blue} (4.4)}\\
{\it \color{gray} Ratio} 		&0.515 {\color{blue} (20)} 		&	0.520 {\color{blue} (21)} 		&	0.490 {\color{blue} (18)} 	&	0.475	 {\color{blue} (17)} 		&	0.498	 {\color{blue} (19)} 		&&0.550 {\color{blue} (16)} 	&	0.461 {\color{blue} (22)} 	&0.461 {\color{blue} (21)} 		&	0.503 {\color{blue} (19)}		&	0.517 {\color{blue} (20)}		&{\color{blue} (19.3)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Gtest 				&0.393 {\color{blue} (6)} 		&0.403 {\color{blue} (7)} 		&0.413 {\color{blue} (8)} 		&0.420 {\color{blue} (3)} 		&	0.435 {\color{blue} (9)} 		&&0.610 {\color{blue} (5)} 	&	0.588 {\color{blue} (10)}	&0.582 {\color{blue} (10)} 	&0.586 {\color{blue} (3)}		&0.563 {\color{blue} (5)}		&{\color{blue} (6.6)}\\
{\color{green} Med}-Gtest 				&0.437 {\color{blue} (13)} 	&0.400 {\color{blue} (5)} 		&0.408 {\color{blue} (5)} 		&0.420 {\color{blue} (3)} 		&	0.453 {\color{blue} (15)} 		&&0.559 {\color{blue} (14)} &	0.590 {\color{blue} (8)} 	&0.600 {\color{blue} (2)} 		&0.580 {\color{blue} (4)}		&0.551 {\color{blue} (10)}	&{\color{blue} (7.9)}\\
{\color{violet} Mod}-Gtest 				&0.448 {\color{blue} (15)} 	&0.383 {\color{blue} (4)} 		&0.398 {\color{blue} (2)} 		&0.428 {\color{blue} (5)} 		&	0.433 {\color{blue} (6)} 		&&0.571 {\color{blue} (12)} &	0.622 {\color{blue} (4)} 	&0.593 {\color{blue} (5)} 		&0.565 {\color{blue} (6)}		&0.551 {\color{blue} (10)}	&{\color{blue} (6.9)}\\
{\color{blue} $\varphi$Pr}-Gtest	&0.450 {\color{blue} (16)} 	&0.445 {\color{blue} (14)} 	&	0.443{\color{blue} (12)}	&0.455 {\color{blue} (11)} 	&	0.433 {\color{blue} (6)} 		&&0.544 {\color{blue} (19)} &	0.555 {\color{blue} (16)}	&0.552 {\color{blue} (12)} 	&0.538 {\color{blue} (13)}	&0.562 {\color{blue} (7)}		&{\color{blue} (12.6)}\\
{\it \color{gray} Gtest} 				&0.440 {\color{blue} (14)} 		&	0.505 {\color{blue} (19)} 		&	0.501 {\color{blue} (21)} 		&	0.486 {\color{blue} (19)} 	&	0.471 {\color{blue} (16)} 		&&	0.542 {\color{blue} (20)} 	&		0.492 {\color{blue} (19)}	&	0.490 {\color{blue} (20)} 	&	0.499 {\color{blue} (21)}		&	0.534 {\color{blue} (16)}		&{\color{blue} (18.5)}\\
\cmidrule{2-6}\cmidrule{8-12}
{\color{red} Exp}-Conf 				&0.405 {\color{blue} (8)} 		&0.415 {\color{blue} (10)} 	&0.453 {\color{blue} (13)} 	&0.455 {\color{blue} (11)} 	&	0.448 {\color{blue} (12)} 		&&0.595 {\color{blue} (8)} 	&	0.587 {\color{blue} (11)}	&0.539 {\color{blue} (15)} 	&0.543 {\color{blue} (12)}	&0.535 {\color{blue} (15)}	&{\color{blue} (11.5)}\\
{\color{green} Med}-Conf 				&0.378 {\color{blue} (2)} 		&0.373 {\color{blue} (2)} 		&0.438 {\color{blue} (11)} 	&0.463 {\color{blue} (15)} 	&	0.435 {\color{blue} (9)} 		&&0.629 {\color{blue} (2)} 	&	0.632 {\color{blue} (2)} 	&0.555 {\color{blue} (11)} 	&0.536 {\color{blue} (15)}	&0.545 {\color{blue} (13)}	&{\color{blue} (8.2)}\\
{\color{violet} Mod}-Conf 				&0.392 {\color{blue} (5)} 		&0.373 {\color{blue} (2)} 		&0.400 {\color{blue} (3)} 		&0.440 {\color{blue} (8)} 		&	0.435 {\color{blue} (9)} 		&&0.606 {\color{blue} (6)} 	&	0.627 {\color{blue} (3)} 	&0.600 {\color{blue} (2)} 		&0.556 {\color{blue} (8)}		&0.563 {\color{blue} (5)}		&{\color{blue} (5.1)}\\
{\color{blue} $\varphi$Pr}-Conf	&0.468 {\color{blue} (19)} 	&0.460 {\color{blue} (15)} 	&	0.495 {\color{blue} (20)} 	&0.505 {\color{blue} (21)} 	&	0.485 {\color{blue} (17)} 		&&0.547 {\color{blue} (18)} &	0.556 {\color{blue} (15)}	&0.519 {\color{blue} (16)} 	&0.507 {\color{blue} (18)}	&0.540 {\color{blue} (14)}	&{\color{blue} (17.3)}\\
{\it \color{gray} Conf} 	&0.455 {\color{blue} (18)} 		&	0.500 {\color{blue} (18)} 	&	0.460 {\color{blue} (15)} 	&	0.464 {\color{blue} (16)} 	&		0.450 {\color{blue} (14)} &&	0.514 {\color{blue} (21)} 	&	0.479 {\color{blue} (20)}	&	0.510 {\color{blue} (17)} 	&	0.498 {\color{blue} (22)}	&	0.519 {\color{blue} (19)}	&{\color{blue} (18.0)}\\
\cmidrule{2-6}\cmidrule{8-12}
Exp-Freq	&0.423 {\color{blue} (10)}	&0.465 {\color{blue} (16)} 	&0.508 {\color{blue} (22)} 	&0.498 {\color{blue} (20)} 	&	0.505 {\color{blue} (22)} 		&&0.579 {\color{blue} (11)} &	0.549 {\color{blue} (17)}	&0.496 {\color{blue} (19)} 	&0.513 {\color{blue} (16)}	&	0.498 {\color{blue} (22)}	&{\color{blue} (17.5)}\\
{\it \color{gray} Freq}		&0.515 {\color{blue} (20)}	&	0.520 {\color{blue} (21)} 	&	0.490 {\color{blue} (18)} 	&	0.475 {\color{blue} (17)} 	&		0.498 {\color{blue} (19)} 		&&	0.550 {\color{blue} (16)} &		0.461 {\color{blue} (21)}	&	0.461 {\color{blue} (21)} 	&	0.503 {\color{blue} (19)}	&	0.517 {\color{blue} (20)}	&{\color{blue} (19.2)}\\
\bottomrule
\end{tabular}
}
\end{table*}



==> table_deletion_game_metric_dnn.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[t]
 \label{tab:nte_deletion_game_table}
{
% \tiny
\centering
\begin{tabular}{lllccccccccc|cc}
\hline
 &  & \multicolumn{10}{c|}{\textbf{Confidence suppression game $\downarrow$}} & \multicolumn{2}{c}{\textbf{Minimality of Saliency}} \\ \hline
\textbf{Dataset} & Method & 10\%  & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 95\%  & \multicolumn{1}{c|}{Sum (\%) $\downarrow$ } & \multicolumn{1}{c}{\left | Variance  \right | \> $\uparrow$} \\ \hline

% \midrule

&Random & 0.69 & 0.73 & 0.75 & 0.77 & 0.79 & 0.81 & 0.83 & 0.85 & 0.90 & 0.95 &\multicolumn{1}{c|}{50} & {0.0001}\\
&RISE \cite{Petsiuk2018RISERI} & 0.92 & 0.92 & 0.93 & 0.93 & 0.93 & 0.94 & 0.94 & 0.94 & 0.94 & 0.94 &\multicolumn{1}{c|}{46} & {0.0001}\\

Computers\cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &1.00 &\multicolumn{1}{c|}{49} & {0.0001} \\

 & LIME \cite{Ribeiro2016WhySI}   & 0.60 & 0.62 & 0.65 & 0.68 & 0.7 & 0.71 & 0.73 & 0.75 & 0.78 & 0.82&\multicolumn{1}{c|}{23} & {0.0001} \\
&SHAP\cite{NIPS2017_7062} &0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 &\multicolumn{1}{c|}{51} & {0.0001}\\

&MP  \cite{Fong2017InterpretableEO}   & 0.75 & 0.76 & 0.78 & 0.81 & 0.81 & 0.82 & 0.82& 0.83 & 0.84 & 0.88 &\multicolumn{1}{c|}{04} & {0.0005}\\
&PERT   &\textbf{0.50} & \textbf{0.50} & \textbf{0.50} &\textbf{0.51} & \textbf{0.51} & \textbf{0.51} & \textbf{0.51} &\textbf{0.51} & \textbf{0.51} & \textbf{0.51} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0017}\\


\midrule





%recheck earthquake indepth for each method

%512
&Random &0.97 & 0.97 & 0.98 & 0.98 & 0.99 & 0.99& 0.99& 0.99& 1.00 &1.00 &\multicolumn{1}{c|}{50} & {0.0001}\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.99 & 0.99 & 0.99& 0.99 & 0.99 & 0.99 & 0.99 & 0.99 &0.99 &0.99 &\multicolumn{1}{c|}{74} & {0.0001}\\
Earthquakes \cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &0.99 &0.99 &0.99 &0.99 &0.99 &0.99 &0.99 &0.99 &1.00 &1.00 &\multicolumn{1}{c|}{61} & {0.0001} \\

 & LIME \cite{Ribeiro2016WhySI}   & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.99 & 0.99 &\multicolumn{1}{c|}{43} & {0.0001}\\
&SHAP\cite{NIPS2017_7062}&0.99 & 0.99 & 0.99 & 0.99 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 &\multicolumn{1}{c|}{51} & {0.0001}\\

&MP  \cite{Fong2017InterpretableEO}   & 0.96 &0.96 &0.96 &0.96 &0.96 & 0.96 & 0.96 & 0.96 & 0.96 & 0.96 &\multicolumn{1}{c|}{04} & {0.0001}\\
&PERT   &\textbf{0.96} & \textbf{0.96} & \textbf{0.96} &\textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} &\textbf{0.96} & \textbf{0.96} & \textbf{0.96} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0039}\\

\midrule

&Random & 0.75 & 0.78 &0.82 &0.84 &0.86 &0.88 &0.89 &0.91 &0.92 &0.95 
&\multicolumn{1}{c|}{50} & 0.0001 \\
&RISE \cite{Petsiuk2018RISERI} & 0.76 & 0.76 & 0.76 & 0.76 & 0.76& 0.76 & 0.77 & 0.77 & 0.77 & 0.78 &\multicolumn{1}{c|}{55} & 0.0001 \\

Ford-A\cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &0.78 &0 &0.79 &0.80 &0.81 &0.82 &0.83 &0.84 &0.84 &0.85 &\multicolumn{1}{c|}{49} & 0.0001 \\

&LIME \cite{Ribeiro2016WhySI}   & 0.71 & 0.75 & 0.78 & 0.81 & 0.83 & 0.84 & 0.86 & 0.87 & 0.89 & 0.92 &\multicolumn{1}{c|}{44} & 0.0001\\
&SHAP\cite{NIPS2017_7062} &0.93 &0.98 &0.98 &0.98 &0.99 &0.99 &0.99 &0.99 &0.99 &0.99 &\multicolumn{1}{c|}{47} & 0.0001 \\

&MP  \cite{Fong2017InterpretableEO}   & 0.66 & 0.67 & 0.70 & 0.72 & 0.75 & 0.77 & 0.78 & 0.81 & 0.83 & 0.87 &\multicolumn{1}{c|}{03} & 0.0010\\
&PERT    &\textbf{0.63} & \textbf{0.64} & \textbf{0.65} &\textbf{0.66} & \textbf{0.66} & \textbf{0.67} & \textbf{0.67} &\textbf{0.68} & \textbf{0.69} & \textbf{0.72} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0012}\\


\midrule
&Random &0.73 & 0.74 & 0.77 & 0.79 & 0.81 & 0.83 & 0.84& 0.85& 0.86 &0.88 &\multicolumn{1}{c|}{50} & {0.0001}\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.73 & 0.81 & 0.85& 0.86 & 0.86 & 0.86 & 0.86 & 0.86 &0.87 &0.87 &\multicolumn{1}{c|}{48} & {0.0001}\\
Ford-B\cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &0.72 &0.73 &0.75 &0.77 &0.80 &0.82 &0.83 &0.84 &0.85 &0.86 &\multicolumn{1}{c|}{49} & {0.0001} \\

& LIME \cite{Ribeiro2016WhySI}   & 0.71 & 0.72 &0.74 &0.77 &0.79 &0.81 &0.81 &0.84 &0.85 &0.87 &\multicolumn{1}{c|}{30} & {0.0001}\\
&SHAP\cite{NIPS2017_7062}&0.71 & 0.72 & 0.74 & 0.75 &0.77  & 0.81 & 0.81 & 0.82 & 0.83 & 0.84 &\multicolumn{1}{c|}{40} & {0.0009}\\

&MP  \cite{Fong2017InterpretableEO}   & 0.71 &0.71 &0.73 &0.74 &0.76 &0.77 &0.78 &0.79 &0.82 &0.83 &\multicolumn{1}{c|}{04} & {0.0008}\\
&PERT   &\textbf{0.70} & \textbf{0.71} & \textbf{0.71} &\textbf{0.72} & \textbf{0.73} & \textbf{0.73} & \textbf{0.74} &\textbf{0.74} & \textbf{0.76} & \textbf{0.77} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0010}\\

\midrule
&Random & 0.21 & 0.27 & 0.35 & 0.41 & 0.49 & 0.61 & 0.72 & 0.89 & 0.93 & 1.00 &\multicolumn{1}{c|}{50} & 0.0001 \\
&RISE \cite{Petsiuk2018RISERI} & 0.15 & 0.15 & 0.26 & 0.35 & 0.45 & 0.55 & 0.63 & 0.91 & 0.91 & 0.95 &\multicolumn{1}{c|}{74} & 0.0001\\

CricketX \cite{conf/kdd/MueenKY11} & LEFTIST \cite{Guillem2019AgnosticLE} & 0.20 & 0.26 & 0.29 & 0.29 & 0.30 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & \multicolumn{1}{c|}{51} & 0.0001 \\
 & LIME \cite{Ribeiro2016WhySI} & 0.14 & 0.19 & 0.23 & 0.26 & 0.29 & 0.31 & 0.34 & 0.37 & 0.41 & 0.48 & \multicolumn{1}{c|}{39} & 0.0001 \\
 & SHAP \cite{NIPS2017_7062} & 0.19 & 0.29 & 0.33 & 0.36 & 0.38 & 0.39 & 0.40 & 0.41 & 0.43 & 0.45 & \multicolumn{1}{c|}{33} & 0.0005 \\
 & MP \cite{Fong2017InterpretableEO} & 0.09 & 0.11 & 0.12 & 0.15 & 0.17 & 0.18 & 0.19 & 0.21 & 0.21 & 0.25 & \multicolumn{1}{c|}{02} & \textbf{0.0040} \\
 & PERT & \textbf{0.06} & \textbf{0.07} & \textbf{0.07} & \textbf{0.08} & \textbf{0.08} & \textbf{0.09} & \textbf{0.10} & \textbf{0.11} & \textbf{0.12} & \textbf{0.15} & \multicolumn{1}{c|}{\textbf{01}} & \textbf{0.0037} \\ 



\midrule
&Random &0.59 & 0.60 & 0.63 & 0.64 & 0.65 & 0.66 & 0.68& 0.70& 0.71 &0.72 &\multicolumn{1}{c|}{50} & {0.0001}\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.52 & 0.57 & 0.66& 0.67 & 0.68 & 0.69 & 0.71 & 0.73 &0.73 &0.75 &\multicolumn{1}{c|}{72} & {0.0001}\\
PTB\cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &0.14 &0.25 &0.45 &0.50 &0.51 &0.55 &0.60 &0.61 &0.62 &0.63 &\multicolumn{1}{c|}{68} & {0.0001} \\

& LIME \cite{Ribeiro2016WhySI}   & 0.51 & 0.60 &0.65 &0.67 &0.70 &0.72 &0.73 &0.73 &0.74 &0.75 &\multicolumn{1}{c|}{45} & {0.0001}\\
&SHAP\cite{NIPS2017_7062}&0.75 & 0.75 & 0.75 & 0.75 & 0.77 & 0.77 & 0.77 & 0.77 & 0.80 & 0.80 &\multicolumn{1}{c|}{58} & {0.0001}\\

&MP  \cite{Fong2017InterpretableEO}   & 0.42 &0.44 &0.46 &0.47 &0.50 &0.52 &0.54 &0.58 &0.60 &0.64 &\multicolumn{1}{c|}{03} & {0.0001}\\
&PERT   &\textbf{0.22} & \textbf{0.29} & \textbf{0.35} &\textbf{38.44} & \textbf{0.45} & \textbf{0.50} & \textbf{0.51} &\textbf{0.52} & \textbf{0.53} & \textbf{0.54} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0018}\\

\midrule
&Random &0.40 & 0.41 & 0.41 & 0.43 & 0.43 & 0.43 & 0.44& 0.45& 0.45 &0.45 &\multicolumn{1}{c|}{50} & {0.0001}\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.40 & 0.40 & 0.40& 0.40 & 0.40 & 0.41 & 0.41 & 0.41 &0.41 &0.41 &\multicolumn{1}{c|}{76} & {0.0001}\\
ECG\cite{UCRArchive} &LEFTIST \cite{Guillem2019AgnosticLE} &0.30 &0.30 &0.30 &0.30 &0.30 &0.31 &0.31 &0.31 &0.31 &0.31 &\multicolumn{1}{c|}{60} & {0.0001} \\

& LIME \cite{Ribeiro2016WhySI}   & 0.71 & 0.72 &0.74 &0.77 &0.79 &0.81 &0.81 &0.84 &0.85 &0.64 &\multicolumn{1}{c|}{42} & {0.0001}\\
&SHAP\cite{NIPS2017_7062}&0.62 & 0.62 & 0.62 & 0.63 & 0.63 & 0.63 & 0.63 & 0.64 & 0.64 & 0.64 &\multicolumn{1}{c|}{64} & {0.0001}\\

&MP  \cite{Fong2017InterpretableEO}   & 0.51 &0.51 &0.51 &0.52 &0.52 &0.52 &0.52 &0.52 &0.53 &0.53 &\multicolumn{1}{c|}{03} & {0.0005}\\
&PERT   &\textbf{0.21} & \textbf{0.21} & \textbf{0.21} &\textbf{0.21} & \textbf{0.21} & \textbf{0.22} & \textbf{0.22} &\textbf{0.22} & \textbf{0.22} & \textbf{0.22} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0034}\\


% \midrule
% &Random &0.79 & 0.82 & 0.86 & 0.87 & 0.87 & 0.88& 0.89& 0.91& 0.91 &0.92\\
% % \midrule
% &RISE \cite{Petsiuk2018RISERI}  & 0.57 & 0.57 & 0.58& 0.59 & 0.59 & 0.59 & 0.61 & 0.61 &0.61 &0.61\\
% Wafer \cite{phdthesis} & LIME \cite{Ribeiro2016WhySI}   &0.69 & 0.73 & 0.82 & 0.82 & 0.83 & 0.84 & 0.84 & 0.86 & 0.86 & 0.88 \\
% &SHAP \cite{NIPS2017_7062}&0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.79 & 0.79 & 0.79 & 0.79 \\
% &MP  \cite{Fong2017InterpretableEO}   & 0.41 &0.47 &0.53 &0.54 &0.55 &0.56 &0.57 &0.58 &0.68 & 0.73\\
% &PERT   &\textbf{0.4} & \textbf{0.4} & \textbf{0.46} &\textbf{0.47} & \textbf{0.48} & \textbf{0.49} & \textbf{0.51} &\textbf{0.53} & \textbf{0.55} & \textbf{0.59}\\

% \midrule
% &Random &0.14 & 0.18 & 0.23 & 0.25 & 0.28 & 0.31& 0.33& 0.36& 0.4 &0.47\\
% % \midrule
% &RISE \cite{Petsiuk2018RISERI}  & 0.11 & 0.12 & 0.14& 0.15 & 0.15 & 0.16 & 0.18 & 0.19 &0.2 &0.23\\
% Cricket-X\cite{conf/kdd/MueenKY11} & LIME \cite{Ribeiro2016WhySI}   & 0.14 &0.19 &0.23 &0.26 &0.29 &0.31 &0.34 &0.37 &0.41 &0.48 \\
% &SHAP\cite{NIPS2017_7062}&0.19 & 0.29 &0.33 & 0.36 & 0.38 & 0.39 & 0.4 & 0.41 & 0.43 & 0.45 \\

% &MP  \cite{Fong2017InterpretableEO}   & 0.09 &0.11 & 0.12 & 0.15 & 0.17 & 0.18 & 0.19 & 0.21 & 0.21 & 0.25\\
% &PERT   &\textbf{0.06} & \textbf{0.07} & \textbf{0.07} &\textbf{0.08} & \textbf{0.08} & \textbf{0.09} & \textbf{0.1} &\textbf{0.11} & \textbf{0.12} & \textbf{0.15}\\


% \midrule
\bottomrule
\end{tabular}
}
\caption{Confidence suppression metric performance with the FCN black-box model. Lower values are better for Saliency sum and Confidence suppression game, Higher values are better for Saliency variance.  $\downarrow$ indicates \textit{the lower the better}. $\uparrow$ indicates \textit{the higher the better}.}% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
\label{tab:dnn_full_confidence}
\end{table*}



==> table_deletion_game_metric_rnn.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[htp]
 \label{tab:rnn_nte_deletion_game_table}
{
% \tiny
\centering
\begin{tabular}{llccccccccccc}
\toprule
% & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
Dataset &Method &10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 95\%\\

\midrule
&Random & 0 & 0 &0 &0 &0 &0 &0 &0 &0 &0\\
&RISE \cite{Petsiuk2018RISERI} & 0.76 & 0.76 & 0.76 & 0.76 & 0.76& 0.76 & 0.77 & 0.77 & 0.77 & 0.78\\

Ford-A\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 0.71 & 0.75 & 0.78 & 0.81 & 0.83 & 0.84 & 0.86 & 0.87 & 0.89 & 0.92 \\
&SHAP\cite{NIPS2017_7062} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\

&CM  \cite{Fong2017InterpretableEO}   & 0.66 & 0.67 & 0.70 & 0.72 & 0.75 & 0.77 & 0.78 & 0.81 & 0.83 & 0.87\\
&NTE    &\textbf{0.63} & \textbf{0.64} & \textbf{0.65} &\textbf{0.66} & \textbf{0.66} & \textbf{0.67} & \textbf{0.67} &\textbf{0.68} & \textbf{0.69} & \textbf{0.72}\\



\midrule
&Random & 0.21 & 0.27 & 0.35 & 0.41 & 0.49 & 0.61 & 0.72 & 0.89 & 0.93 & 1\\
&RISE \cite{Petsiuk2018RISERI} & 0.15 & 0.15 & 0.26 & 0.35 & 0.45 & 0.55 & 0.63 & 0.91 & 0.91 & 0.95\\

Gun-Point\cite{conf/sdm/RatanamahatanaK05} & LIME \cite{Ribeiro2016WhySI}   & 0.18 & 0.24 & 0.31 & 0.37 & 0.46 & 0.56 & 0.67 & 0.83 & 0.87 & 0.95 \\
&SHAP\cite{NIPS2017_7062} &0.33 & 0.42 & 0.43 & 0.52 & 0.54 & 0.54 & 0.58 & 1 & 1 & 1\\

&CM  \cite{Fong2017InterpretableEO}   & 0.14 & 0.16 & 0.36 & 0.51 & 0.61 & 0.68 & 0.76& 0.92 & 0.95 & 1\\
&NTE    &\textbf{0.13} & \textbf{0.14} & \textbf{0.14} &\textbf{0.16} & \textbf{0.18} & \textbf{0.2} & \textbf{0.24} &\textbf{0.72} & \textbf{0.73} & \textbf{0.77}\\



\midrule
&Random & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
&RISE \cite{Petsiuk2018RISERI} & 0.92 & 0.92 & 0.93 & 0.93 & 0.93 & 0.94 & 0.94 & 0.94 & 0.94 & 0.94\\

Computers\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 0.6 & 0.62 & 0.65 & 0.68 & 0.7 & 0.71 & 0.73 & 0.75 & 0.78 & 0.82 \\
&SHAP\cite{NIPS2017_7062} &1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\

&CM  \cite{Fong2017InterpretableEO}   & 0.75 & 0.76 & 0.78 & 0.81 & 0.81 & 0.82 & 0.82& 0.83 & 0.84 & 0.88\\
&NTE    &\textbf{0.5} & \textbf{0.5} & \textbf{0.5} &\textbf{0.51} & \textbf{0.51} & \textbf{0.51} & \textbf{0.51} &\textbf{0.51} & \textbf{0.51} & \textbf{0.51}\\


\midrule

%recheck earthquake indepth for each method

%512
&Random &0 & 0 & 0 & 0 & 0 & 0& 0& 0& 0 &0\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 1 & 1 & 1& 1 & 1 & 1 & 1 & 1 &1 &1\\
Earthquakes \cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.99 & 0.99\\
&SHAP\cite{NIPS2017_7062}&1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\

&CM  \cite{Fong2017InterpretableEO}   & 0.96 &0.96 &0.96 &0.96 &0.96 & 0.96 & 0.96 & 0.96 & 0.96 & 0.96\\
&NTE    &\textbf{0.96} & \textbf{0.96} & \textbf{0.96} &\textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} &\textbf{0.96} & \textbf{0.96} & \textbf{0.96}\\


\midrule
&Random &0.73 & 0.74 & 0.77 & 0.79 & 0.81 & 0.83 & 0.84& 0.85& 0.86 &0.88\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.73 & 0.81 & 0.85& 0.86 & 0.86 & 0.86 & 0.86 & 0.86 &0.87 &0.87\\
Ford-B\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 0.71 & 0.72 &0.74 &0.77 &0.79 &0.81 &0.81 &0.84 &0.85 &0.87 \\
&SHAP\cite{NIPS2017_7062}&0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

&CM  \cite{Fong2017InterpretableEO}   & 0.71 &0.71 &0.73 &0.74 &0.76 &0.77 &0.78 &0.79 &0.82 &0.83\\
&NTE    &\textbf{0.70} & \textbf{0.71} & \textbf{0.71} &\textbf{0.72} & \textbf{0.73} & \textbf{0.73} & \textbf{0.74} &\textbf{0.74} & \textbf{0.76} & \textbf{0.77}\\


\midrule
&Random &0.79 & 0.82 & 0.86 & 0.87 & 0.87 & 0.88& 0.89& 0.91& 0.91 &0.92\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.57 & 0.57 & 0.58& 0.59 & 0.59 & 0.59 & 0.61 & 0.61 &0.61 &0.61\\
Wafer \cite{phdthesis} & LIME \cite{Ribeiro2016WhySI}   &0.69 & 0.73 & 0.82 & 0.82 & 0.83 & 0.84 & 0.84 & 0.86 & 0.86 & 0.88 \\
&SHAP \cite{NIPS2017_7062}&0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.79 & 0.79 & 0.79 & 0.79 \\
&CM  \cite{Fong2017InterpretableEO}   & 0.41 &0.47 &0.53 &0.54 &0.55 &0.56 &0.57 &0.58 &0.68 & 0.73\\
&NTE    &\textbf{0.4} & \textbf{0.4} & \textbf{0.46} &\textbf{0.47} & \textbf{0.48} & \textbf{0.49} & \textbf{0.51} &\textbf{0.53} & \textbf{0.55} & \textbf{0.59}\\

\midrule
&Random &0.14 & 0.18 & 0.23 & 0.25 & 0.28 & 0.31& 0.33& 0.36& 0.4 &0.47\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 0.11 & 0.12 & 0.14& 0.15 & 0.15 & 0.16 & 0.18 & 0.19 &0.2 &0.23\\
Cricket-X\cite{conf/kdd/MueenKY11} & LIME \cite{Ribeiro2016WhySI}   & 0.14 &0.19 &0.23 &0.26 &0.29 &0.31 &0.34 &0.37 &0.41 &0.48 \\
&SHAP\cite{NIPS2017_7062}&0.19 & 0.29 &0.33 & 0.36 & 0.38 & 0.39 & 0.4 & 0.41 & 0.43 & 0.45 \\

&CM  \cite{Fong2017InterpretableEO}   & 0.09 &0.11 & 0.12 & 0.15 & 0.17 & 0.18 & 0.19 & 0.21 & 0.21 & 0.25\\
&NTE    &\textbf{0.06} & \textbf{0.07} & \textbf{0.07} &\textbf{0.08} & \textbf{0.08} & \textbf{0.09} & \textbf{0.1} &\textbf{0.11} & \textbf{0.12} & \textbf{0.15}\\


% \midrule
\bottomrule
\end{tabular}
}
\caption{Confidence-Suppression Metric performance for all datasets. Lower values are better.}% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
\end{table*}



==> table_deletion_game_metric_time_steps.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[htp]
 \label{tab:nte_deletion_game_table_raw}
{
% \tiny
\centering
\begin{tabular}{llccccccccccc}
\toprule
% & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
Dataset &Method &10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 95\%\\

\midrule
&Random & 1 & 1 &1 &1 &1 &1 &1 &1 &1 &1\\
&RISE \cite{Petsiuk2018RISERI} & 380 & 382 & 382 & 384 & 384& 385 & 387 & 388 & 389 & 392\\

Ford-A\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 356 & 375 & 393 & 408 & 416 & 423 & 431 & 439 & 448 & 461 \\
&SHAP\cite{NIPS2017_7062} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\

&CM  \cite{Fong2017InterpretableEO}   & 333 & 338 & 352 & 363 & 375 & 386 & 394 & 402 & 416 & 437\\
&NTE    &\textbf{317} & \textbf{32} & \textbf{327} &\textbf{330} & \textbf{332} & \textbf{335} & \textbf{337} &\textbf{341} & \textbf{349} & \textbf{362}\\



\midrule
&Random & 32 & 41 & 53 & 62 & 74 & 91 & 108 & 134 & 140 & 152\\
&RISE \cite{Petsiuk2018RISERI} & 22 & 23 & 39 & 52 & 68 & 82 & 94 & 136 & 137 & 142\\

Gun-Point\cite{conf/sdm/RatanamahatanaK05} & LIME \cite{Ribeiro2016WhySI}   & 28 & 37 & 47 & 56 & 69 & 84 & 101 & 125 & 131 & 143 \\
&SHAP\cite{NIPS2017_7062} &50 & 64 & 74 & 78 & 81 & 82 & 88 & 152 & 152 & 152\\

&CM  \cite{Fong2017InterpretableEO}   & 21 & 24 & 54 & 76 & 92 & 102 & 114& 139 & 143 & 151\\
&NTE    &\textbf{20} & \textbf{21} & \textbf{22} &\textbf{24} & \textbf{28} & \textbf{30} & \textbf{37} &\textbf{109} & \textbf{110} & \textbf{116}\\



\midrule
&Random & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
&RISE \cite{Petsiuk2018RISERI} & 663 & 666 & 669 & 672 & 673 & 673 & 674 & 674 & 677 & 678\\

Computers\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 432 & 452 & 475 & 490 & 504 & 517 & 530 & 542 & 562 & 594 \\
&SHAP\cite{NIPS2017_7062} &720 & 720 & 720 & 720 & 720 & 720 & 720 & 720 & 720 & 720\\

&CM  \cite{Fong2017InterpretableEO}   & 540 & 553 & 568 & 579 & 585 & 591 & 597& 601 & 611 & 639\\
&NTE    &\textbf{360} & \textbf{360} & \textbf{361} &\textbf{362} & \textbf{362} & \textbf{363} & \textbf{363} &\textbf{364} & \textbf{365} & \textbf{367}\\




\midrule

%recheck earthquake indepth for each method

&Random &0 & 0 & 0 & 0 & 0 & 0& 0& 0& 0 &0\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 512 & 512 & 512& 512 & 512 & 512 & 512 & 512 &512 &512\\
Earthquakes \cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 501 & 503 & 504 & 504 & 505 & 506 & 507 & 507 & 508 & 509 \\
&SHAP\cite{NIPS2017_7062}&512 & 512 & 512 & 512 & 512 & 512 & 512 & 512 & 512 & 512 \\

&CM  \cite{Fong2017InterpretableEO}   & 495 &495 & 495 & 495 & 495 & 495 & 495 & 495 & 495 & 496\\
&NTE    &\textbf{495} & \textbf{495} & \textbf{495} &\textbf{495} & \textbf{495} & \textbf{495} & \textbf{495} &\textbf{495} & \textbf{495} & \textbf{495}\\


\midrule
&Random &365 & 372 & 385 & 397 & 406 & 596 & 422& 428& 434 &442\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 365 & 405 & 426& 431 & 432 & 433 & 433 & 433 &437 &438\\
Ford-B\cite{Eamonnwebsite} & LIME \cite{Ribeiro2016WhySI}   & 354 & 361 & 374 & 386 & 396 & 406 & 414 & 421 & 428 & 436 \\
&SHAP\cite{NIPS2017_7062}&0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\

&CM  \cite{Fong2017InterpretableEO}   & 352 &356 & 366 & 372 & 383 & 388 & 392 & 398 & 410 & 416\\
&NTE    &\textbf{354} & \textbf{356} & \textbf{358} &\textbf{364} & \textbf{366} & \textbf{368} & \textbf{370} &\textbf{374} & \textbf{380} & \textbf{386}\\


\midrule
&Random &121 & 125 & 131 & 133 & 133 & 135& 136& 137& 138 &141\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 87 & 88 & 89& 90 & 91 & 91 & 92 & 92 &92 &93\\
Wafer \cite{phdthesis} & LIME \cite{Ribeiro2016WhySI}   & 106 & 111 & 125 & 126 & 127 & 128 & 129 & 131 & 132 & 134 \\
&SHAP \cite{NIPS2017_7062}&119 & 119 & 119 & 119 & 119 & 120 & 121 & 121 & 121 & 121 \\

&CM  \cite{Fong2017InterpretableEO}   & 62 &72 & 82 & 83 & 84 & 86 & 87 & 89 & 104 & 112\\
&NTE    &\textbf{61} & \textbf{62} & \textbf{70} &\textbf{72} & \textbf{74} & \textbf{75} & \textbf{78} &\textbf{82} & \textbf{84} & \textbf{90}\\




\midrule
&Random &41 & 55 & 69 & 77 & 84 & 92& 98& 108& 119 &142\\
% \midrule
&RISE \cite{Petsiuk2018RISERI}  & 34 & 37 & 41& 44 & 46 & 49 & 53 & 56 &60 &69\\
Cricket-X\cite{conf/kdd/MueenKY11} & LIME \cite{Ribeiro2016WhySI}   & 41 & 56 & 70 & 78 & 87 & 94 & 102 & 111 & 122 & 143 \\
&SHAP\cite{NIPS2017_7062}&56 & 87 & 99 & 108 & 112 & 116 & 119 & 123 & 129 & 136 \\

&CM  \cite{Fong2017InterpretableEO}   & 26 &31 & 37 & 45 & 51 & 54 & 58 & 62 & 62 & 76\\
&NTE    &\textbf{20} & \textbf{20} & \textbf{22} &\textbf{24} & \textbf{25} & \textbf{27} & \textbf{29} &\textbf{32} & \textbf{36} & \textbf{44}\\


% \midrule
\bottomrule
\end{tabular}
}
\caption{Confidence Suppression Game Metrics: Percentage of Black Box Confidence Suppression Vs Number of Time Steps. \tnote{Please normalize these numbers by the number of timesteps so that it's a proportion of timesteps instead of just an integer}}
\end{table*}



==> table_deletion_game_short_normalized.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


% \begin{table*}[htp]
%  \label{tab:nte_deletion_game_short_norm}
% {
% % \tiny
% \centering
% \begin{tabular}{llccccccccccc}
% \toprule
% % & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
% Dataset &Method &10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 95\%\\
% \midrule
% &Random &0.79 & 0.82 & 0.86 & 0.87 & 0.87 & 0.88& 0.89& 0.91& 0.91 &0.92\\
% % \midrule
% &RISE \cite{Petsiuk2018RISERI}  & 0.57 & 0.57 & 0.58& 0.59 & 0.59 & 0.59 & 0.61 & 0.61 &0.61 &0.61\\
% Wafer \cite{phdthesis} & LIME \cite{Ribeiro2016WhySI}   &0.69 & 0.73 & 0.82 & 0.82 & 0.83 & 0.84 & 0.84 & 0.86 & 0.86 & 0.88 \\
% &SHAP \cite{NIPS2017_7062}&0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.79 & 0.79 & 0.79 & 0.79 \\
% &CM  \cite{Fong2017InterpretableEO}   & 0.41 &0.47 &0.53 &0.54 &0.55 &0.56 &0.57 &0.58 &0.68 & 0.73\\
% &NTE    &\textbf{0.4} & \textbf{0.4} & \textbf{0.46} &\textbf{0.47} & \textbf{0.48} & \textbf{0.49} & \textbf{0.51} &\textbf{0.53} & \textbf{0.55} & \textbf{0.59}\\

% \midrule
% &Random &0.14 & 0.18 & 0.23 & 0.25 & 0.28 & 0.31& 0.33& 0.36& 0.4 &0.47\\
% % \midrule
% &RISE \cite{Petsiuk2018RISERI}  & 0.11 & 0.12 & 0.14& 0.15 & 0.15 & 0.16 & 0.18 & 0.19 &0.2 &0.23\\
% Cricket-X\cite{conf/kdd/MueenKY11} & LIME \cite{Ribeiro2016WhySI}   & 0.14 &0.19 &0.23 &0.26 &0.29 &0.31 &0.34 &0.37 &0.41 &0.48 \\
% &SHAP\cite{NIPS2017_7062}&0.19 & 0.29 &0.33 & 0.36 & 0.38 & 0.39 & 0.4 & 0.41 & 0.43 & 0.45 \\

% &CM  \cite{Fong2017InterpretableEO}   & 0.09 &0.11 & 0.12 & 0.15 & 0.17 & 0.18 & 0.19 & 0.21 & 0.21 & 0.25\\
% &NTE    &\textbf{0.06} & \textbf{0.07} & \textbf{0.07} &\textbf{0.08} & \textbf{0.08} & \textbf{0.09} & \textbf{0.1} &\textbf{0.11} & \textbf{0.12} & \textbf{0.15}\\


% % \midrule
% \bottomrule
% \end{tabular}
% }
% \caption{Confidence-Suppression Metric performance for all datasets. Lower values are better.}% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
% \end{table*}


\begin{table*}[]
\centering
\begin{tabular}{lllccccccccc|cc}
\hline
 &  & \multicolumn{10}{c|}{\textbf{Confidence suppression game $\downarrow$}} & \multicolumn{2}{c}{\textbf{Minimality of Saliency}} \\ \hline
\textbf{Dataset} & Method & 10\%  & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 95\%  & \multicolumn{1}{c|}{Sum (\%) $\downarrow$ } & |Variance| \> $\uparrow$ \\ \hline
 & Random & 0.79 & 0.82 & 0.86 & 0.87 & 0.87 & 0.88 & 0.89 & 0.91 & 0.91 & 0.92 & \multicolumn{1}{c|}{50} & 0.0016 \\
 & RISE \cite{Petsiuk2018RISERI} & 0.57 & 0.57 & 0.58 & 0.59 & 0.59 & 0.59 & 0.61 & 0.61 & 0.61 & 0.61 & \multicolumn{1}{c|}{82} & 0.0001 \\
& LEFTIST \cite{Guillem2019AgnosticLE} & 0.56 & 0.57 & 0.58 & 0.58 & 0.58 & 0.58 & 0.58 & 0.58 & 0.58 & 0.59 & \multicolumn{1}{c|}{78} & 0.0001 \\
 
\textsc{Wafer} \cite{phdthesis} & LIME \cite{Ribeiro2016WhySI} & 0.69 & 0.73 & 0.82 & 0.82 & 0.83 & 0.84 & 0.84 & 0.86 & 0.86 & 0.88 & \multicolumn{1}{c|}{42} & 0.0001 \\
 
 & SHAP \cite{NIPS2017_7062} & 0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.78 & 0.79 & 0.79 & 0.79 & 0.79 & \multicolumn{1}{c|}{52} & 0.0004 \\
 & MP \cite{Fong2017InterpretableEO} & 0.41 & 0.47 & 0.53 & 0.54 & 0.55 & 0.56 & 0.57 & 0.58 & 0.68 & 0.73 & \multicolumn{1}{c|}{06} & 0.0041 \\
 & PERT & \textbf{0.40} & \textbf{0.40} & \textbf{0.46} & \textbf{0.47} & \textbf{0.48} & \textbf{0.49} & \textbf{0.51} & \textbf{0.53} & \textbf{0.55} & \textbf{0.59} & \multicolumn{1}{c|}{\textbf{01}} & \textbf{0.0153} \\ \hline
 
 
 & Random & 0.14 & 0.18 & 0.23 & 0.25 & 0.28 & 0.31 & 0.33 & 0.36 & 0.40 & 0.47 & \multicolumn{1}{c|}{50} & 0.0001 \\
 & RISE \cite{Petsiuk2018RISERI} & 0.11 & 0.12 & 0.14 & 0.15 & 0.15 & 0.16 & 0.18 & 0.19 & 0.20 & 0.23 & \multicolumn{1}{c|}{57} & 0.0001 \\

&LEFTIST \cite{Guillem2019AgnosticLE} &0.14 &0.00 &0.14 &0.15 &0.19 &0.35 &0.46 &0.71 &0.71 &0.72 &\multicolumn{1}{c|}{63} & 0.0001 \\

\textsc{GunPoint} \cite{conf/sdm/RatanamahatanaK05} & LIME \cite{Ribeiro2016WhySI}   & 0.18 & 0.24 & 0.31 & 0.37 & 0.46 & 0.56 & 0.67 & 0.83 & 0.87 & 0.95&\multicolumn{1}{c|}{36} & 0.0005 \\
&SHAP\cite{NIPS2017_7062} &0.33 & 0.42 & 0.43 & 0.52 & 0.54 & 0.54 & 0.58 & 1.00 & 1.00 & 1.00 &\multicolumn{1}{c|}{60} & 0.0005\\

&MP  \cite{Fong2017InterpretableEO}   & 0.14 & 0.16 & 0.36 & 0.51 & 0.61 & 0.68 & 0.76& 0.92 & 0.95 & 1.00 &\multicolumn{1}{c|}{10} & 0.0035\\
&PERT   &\textbf{0.13} & \textbf{0.14} & \textbf{0.14} &\textbf{0.16} & \textbf{0.18} & \textbf{0.20} & \textbf{0.24} &\textbf{0.72} & \textbf{0.73} & \textbf{0.77} &\multicolumn{1}{c|}{\textbf{02}} & \textbf{0.0100}\\
\midrule 

 \end{tabular}
\caption{Confidence suppression metric performance for two key datasets with the FCN black-box model. Lower values are better for Saliency sum and Confidence suppression game, Higher values are better for Saliency variance. $\downarrow$ indicates \textit{the lower the better}. $\uparrow$ indicates \textit{the higher the better}.}% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
\label{table2}
\label{tab:dnn_nte_confidence}
\end{table*}

==> table_deletion_game_short_normalized_cikm.tex <==

\begin{table*}[]
\centering
\begin{tabular}{lllccc|cc}
\hline
 &  & \multicolumn{4}{c|}{\textbf{Confidence suppression game $\downarrow$}} & \multicolumn{2}{c}{\textbf{Minimality of Saliency}} \\ \hline
\textbf{Dataset} & Method & 60\% & 80\% & 90\% & 95\%  & \multicolumn{1}{c|}{Sum (\%) $\downarrow$ } & \|Variance\| \> $\uparrow$ \\ \hline

 
 & RISE  & 0.33 & 0.39 & 0.41 & 0.45 & \multicolumn{1}{c|}{46} & 0.019 \\
 
 & SHAP  & 0.24 & 0.30 & 0.35 & 0.44 & \multicolumn{1}{c|}{49} & 0.012 \\
 
 \textsc{ACSF} & LIME    & 0.33 & 0.36 & 0.38 & 0.42 & \multicolumn{1}{c|}{48} & 0.021 \\
 
%  41
 & CM  & 0.24 & 0.27 & 0.32 & 0.46 & \multicolumn{1}{c|}{43} & 0.036\\
 
 & PERT & 0.25 & 0.27 & 0.29 & 0.32 & \multicolumn{1}{c|}{41} & 0.011 \\
 
 & MUX &  \textbf{0.18} & \textbf{0.24} & \textbf{0.27} & \textbf{0.31} & \multicolumn{1}{c|}{\textbf{37}} & \textbf{0.015} \\ \hline
 
 \bottomrule
 \end{tabular}
\caption{Confidence suppression metric performance for datasets with the FCN black-box model. Lower values are better for Saliency sum and Confidence suppression game, Higher values are better for Saliency variance. $\downarrow$ indicates \textit{the lower the better}. $\uparrow$ indicates \textit{the higher the better}.} 
% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
\label{table2}
\label{tab:dnn_nte_confidence_cikm}
\end{table*}





==> table_deletion_game_short_normalized_rnn.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lllccc|cc}
\hline
 &  & \multicolumn{4}{c|}{\textbf{Confidence suppression game $\downarrow$}} & \multicolumn{2}{c}{\textbf{Minimality of Saliency}} \\ \hline
\textbf{Dataset} & Method & 60\% & 80\% & 90\% & 95\%  & \multicolumn{1}{c|}{Sum (\%) $\downarrow$ } & \|Variance\| \> $\uparrow$ \\ \hline

 
 & RISE  & 0.51 & 0.52 & 0.52 & 0.52 & \multicolumn{1}{c|}{122} & 0.001 \\
 
 & SHAP  & 0.79 & 0.79 & 0.79 & 0.79 & \multicolumn{1}{c|}{208} & 0.007 \\
 
 \textsc{Trace} & LIME    & 0.74 & 0.74 & 0.74 & 0.74 & \multicolumn{1}{c|}{163} & 0.007 \\
 
%  41
 & CM  & 0.42 & 0.45 & 0.45 & 0.46 & \multicolumn{1}{c|}{35} & 0.006\\
 
 & PERT & 0.23 & 0.25 & 0.26 & 0.31 & \multicolumn{1}{c|}{42} & 0.006 \\
 
 & MUX &  \textbf{0.23} & \textbf{0.24} & \textbf{0.25} & \textbf{0.30} & \multicolumn{1}{c|}{\textbf{22}} & \textbf{0.006} \\ \hline
 
 \bottomrule
 \end{tabular}
\caption{Confidence suppression metric performance for datasets with the RNN black-box model. Lower values are better for Saliency sum and Confidence suppression game, Higher values are better for Saliency variance. $\downarrow$ indicates \textit{the lower the better}. $\uparrow$ indicates \textit{the higher the better}.} 
% : Percentage of Black Box Confidence Suppression Vs Normalized Number of Time Steps.}
\label{table2}
\label{tab:rnn_nte_confidence_cikm}
\end{table*}

==> table_dnn_nte_auc.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[hbt!]
 
{
% \tiny
\centering
\begin{tabular}{lccccccccc}
\toprule
% & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
\multirow{2.5}{*}{\textbf{Methods}} & \multicolumn{9}{c}{\textbf{Datasets}}\\
\cmidrule{2-10}
 &\textsc{Wafer} & \textsc{GunPoint} & \textsc{Computers} & \textsc{Earthquakes} & \textsc{FordA} & \textsc{FordB} & \textsc{CricketX} & \textsc{PTB}  & \textsc{ECG}\\
\midrule
Random & -0.02 (.01) & 0.02 (.01) & 0.01 (.01) & -0.01 (.01) & -0.03 (.01) & -0.01(.01) &-0.01 (.01) & 0.06 (.04) & 0.01 (.06) \\
RISE \cite{Petsiuk2018RISERI}  & \ 0.22 (.01) & 0.16 (.01) &-0.01 (.02) & 0.23  (.05) & 0.15 (.02) & 0.11 (.01) &0.42  (.01) & 0.07    (.05) & 0.14 (.07)\\
LEFTIST \cite{Guillem2019AgnosticLE}& 0.53 (.02) & 0.15 (.03) & -0.16 (.01) & 0.15 (.03)  & 0.16 (.01) & 0.15 (.01) &-0.01 (.01) &0.51 (.01) & 0.55 (.01)\\
\midrule
LIME \cite{Ribeiro2016WhySI}   & 0.06 (.01) & \ 0.10 (.01) &0.06  (.03) &-0.01  (.01) & 0.01 (.02) & 0.01 (.01) &-0.01 (.01) & 0.18 (.07) & 0.09 (.06)\\
\midrule
SHAP \cite{NIPS2017_7062}  & -0.19 (.01) & -0.01 (.01) & ~0.10   (.01) & 0.71  (.03) & 0.23 (.01) &-0.17 (.01) &0.09  (.01) &-0.15  (.01) & -0.11 (.09) \\
\midrule
MP  \cite{Fong2017InterpretableEO}   & 0.49 (.01) & ~0.03  (.01) &0.15 (.01) & 0.33  (.01) & 0.48 (.01) & 0.37 (.01) &0.43  (.01) & 0.33 (.01) & -0.16 (.00)  \\
% MSE & 0.60 (.01) & 0.48 (.01) &0.70 (.01) & 0.60 (.03)  & 0.51 (.01) & 0.49 (.02) &0.50 (.03)  &0.50 (.01) & 0.47 (.02) \\

PERT    &\textbf{0.74 (.01)} & \textbf{0.56 (.01)} & \textbf{0.95 (.01)} &\textbf{0.93 (.01)} & \textbf{0.83 (.01)} & \textbf{0.82 (.01)} & \textbf{0.69 (.01)} & \textbf{0.58 (.01)} & \textbf{0.60 (.01)}\\
\bottomrule
\end{tabular}
}
\caption{Performance of the AUC-difference metric with the FCN black-box model. Parentheses indicate $\sigma$. Compared methods are separated into four groups: Random perturbation, linear surrogate model, game theory method, and learned perturbations.} 
\label{tab:nte_auc_table}
\vspace{-7mm}
\end{table*}

% \label{tab:auc}



==> table_nte.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[hbt!]
\caption{Average difference between Insertion and Deletion AUC metrics across 5 runs over 7 real datasets from multiple methods \tnote{I think I've mentioned this before, but let's use parentheses for standard deviation. Also seems like there's no need for a "Model" column. Take a look at tables from other papers to figure out how to structure this. I think I've voted a couple of times for there to be one row per method and one column per dataset. It should take up two columns. Also let's not go over two decimals of precision. (.06) instead of (.0615) because we can't claim accuracy on 3-4 decimals, it hasn't been replicated enough. I changed the formatting on NTE for Ford-A to show how it should look.} }
\label{tab:nte_auc_table}
{
\tiny
\centering
\begin{tabular}{lrrrr}
\toprule
% & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
Dataset & Model & Method & Avg. & Stddev\\
\midrule
{\color{violet} Ford-A} 
&DNN  	&Random &-0.0309    & 0.0615\\
&DNN   &RISE   & 0.1593 	& 0.0129\\
&DNN   &LIME   & 0.0104 	& 0.0158\\
&DNN   &SHAP   & 0.2312 	& 0.0115\\
&DNN   &CM     & 0.4838 	& 0.0062\\
&DNN   &\color{blue}NTE    & \textbf{0.70 (.01)} 	& 0.0058 		
\\
\midrule
{\color{violet} Gun-Point} 
&DNN  	&Random & 0.0267    & 0.0111\\
&DNN   &RISE   & 0.1655  	& 0.0068\\
&DNN   &LIME   & 0.1059 	& 0.0050\\
&DNN   &SHAP   &-0.0046 	& 0.0007\\
&DNN   &CM     & 0.0227 	& 0.0005\\
&DNN   &\color{blue}NTE    & \color{blue}0.5557 	& 0.0049 		
\\
\midrule
{\color{violet} Computers} 
&DNN  	&Random & 0.0028    & 0.0233\\
&DNN   &RISE   &-0.0167 	& 0.0587\\
&DNN   &LIME   & 0.0558 	& 0.0238\\
&DNN   &SHAP   & 0.0944 	& 0.0115\\
&DNN   &CM     & 0.1460 	& 0.0007\\
&DNN   &\color{blue}NTE    &\color{blue} 0.9261 	& 0.0037 		
\\
\midrule
{\color{violet} Earthquakes} 
&DNN  	&Random &-0.0125    & 0.0117\\
&DNN   &RISE   & 0.2280 	& 0.0456\\
&DNN   &LIME   &-0.0007 	& 0.0064\\
&DNN   &SHAP   & 0.7123 	& 0.0355\\
&DNN   &CM     & 0.3382 	& 0.0002\\
&DNN   &\color{blue}NTE    & \color{blue}0.7219 	& 0.0089 		
\\
\midrule
{\color{violet} Ford-B} 
&DNN  	&Random &-0.0068    & 0.0194\\
&DNN   &RISE   & 0.1090 	& 0.0242\\
&DNN   &LIME   & 0.0113 	& 0.0115\\
&DNN   &SHAP   &-0.1714 	& 0.0005\\
&DNN   &CM     & 0.3720 	& 0.0096\\
&DNN   &\color{blue}NTE    &\color{blue} 0.6043 	& 0.0114 		
\\
\midrule
{\color{violet} Wafer} 
&DNN  	&Random &-0.0176    & 0.0092\\
&DNN   &RISE   & 0.2182 	& 0.0048\\
&DNN   &LIME   & 0.0575 	& 0.0093\\
&DNN   &SHAP   &-0.1920 	& 0.0037\\
&DNN   &CM     & 0.4917 	& 0.0036\\
&DNN   &\color{blue}NTE    &\color{blue} 0.4979 	& 0.0108 		
\\
\midrule
{\color{violet} Cricket-X} 
&DNN  	&Random &-0.0030    & 0.0094\\
&DNN   &RISE   & 0.4223 	& 0.0016\\		
&DNN   &LIME   &-0.0106 	& 0.0092\\		
&DNN   &SHAP   & 0.0945 	& 0.0048\\		
&DNN   &CM     & 0.4276 	& 0.0089\\ 		
&DNN   &\color{blue}NTE    &\color{blue} 0.6460 	& 0.0043 		
\\
\bottomrule
\end{tabular}
}
\end{table*}



==> table_rnn_nte_auc.tex <==
%-------------------------------------------------------
% Table of Major Result 
% The goal is to show the proposed method outperform all base methods. 
% Key points:
%   1) if with space, show both mean and standard deviation 
%   2) highlight the major message in the table, make it easier for reviewers to understand.
%   3) show a lot of numbers. also to show the efforts to reviewers,  make sure we have done enough works. 
%
% For more details, see here: http://dmkd.cs.wpi.edu/xkong/tutorials/blob/master/paper_writing/readme.md
%-------------------------------------------------------


%-------------------------------------------------------
% here is an example to fill the space before you finish your own table
%-------------------------------------------------------


\begin{table*}[t]
 {
% \tiny
\centering
\begin{tabular}{lccccccccc}
\toprule
% & \multicolumn{5}{c}{Data set}&{Model}&{Method}&Avg.&Stddev\\
\multirow{2.5}{*}{\textbf{Methods}} & \multicolumn{9}{c}{\textbf{Datasets}}\\
\cmidrule{2-10}
 &\textsc{Wafer} & \textsc{GunPoint} & \textsc{Computers} & \textsc{Earthquakes} & \textsc{FordA} & \textsc{FordB} & \textsc{CricketX} & \textsc{PTB}  & \textsc{ECG}\\
\midrule
Random & 0.01 (.01) & 0.03 (.01) & 0.01 (.01) & 0.04 (.01) & 0.01 (.01) & 0.01(.01) &-0.01 (.01) & 0.07 (.04) & 0.01 (.06) \\
%TODO 
RISE \cite{Petsiuk2018RISERI}  & \ 0.13 (.01) & 0.10 (.01) &-0.01 (.02) & 0.23  (.05) & 0.15 (.01) & 0.11 (.02) &0.42  (.01) & 0.10    (.05) & 0.19 (.07)\\
%TODO
LEFTIST \cite{Guillem2019AgnosticLE}& 0.16 (.01) & 0.15 (.03) & -0.16 (.01) & 0.53 (.03)  & 0.15 (.02) & 0.15 (.01) &-0.10 (.01) & 0.42 (.01) & 0.51 (.01)\\
\midrule

LIME \cite{Ribeiro2016WhySI}   & 0.07 (.01) & \ 0.02 (.01) &0.05  (.03) & -0.02  (.01) & 0.01 (.01) & 0.01 (.01) & 0.03 (.01) & 0.12 (.07) & 0.09 (.06)\\
\midrule
SHAP \cite{NIPS2017_7062}  & -0.15 (.01) & -0.01 (.01) & ~0.10   (.01) & \textbf{0.80  (.03)} & 0.23 (.01) &-0.17 (.01) &0.30  (.01) &-0.14  (.01) & 0.08 (.09) \\
\midrule
MP  \cite{Fong2017InterpretableEO}   & 0.55 (.01) & ~0.02  (.01) &0.16  (.01) & 0.30  (.01) & 0.47 (.01) & 0.39 (.01) &0.23  (.01) & 0.30 (.01) & -0.15 (.01)  \\
% MSE & 0.60 (.01) & 0.48 (.01) &0.70 (.01) & 0.60 (.03)  & 0.51 (.01) & 0.49 (.02) &0.50 (.03)  &0.50 (.01) & 0.47 (.02) \\

PERT    &\textbf{0.78 (.01)} & \textbf{0.48 (.01)} & \textbf{0.92 (.01)} &\textbf{0.82 (.01)} & \textbf{0.70 (.01)} & \textbf{0.70 (.01)} & \textbf{0.68 (.01)} & \textbf{0.52 (.01)} & \textbf{0.57 (.01)}\\
\bottomrule
\end{tabular}
}
\caption{Average performance of the AUC-difference metric with the RNN black-box model.} % Parentheses indicate $\sigma$. The four groups of methods are indicated by horizontal lines: Random perturbation, linear surrogate model, game theory method, and learn to perturb.} 
\label{tab:rnn_nte_auc_table}
\end{table*}\label{tab:rnn_auc}

==> valid_points.tex <==
% \sout{

% Important Points:


% 0.	When the length of time steps is shorter than RISE performs better and it deteriorates when the time series length increases. We see this in AUC metrics across WAFER and Ford B datasets.
% 1.	For NTE Time-series length doesn’t matter.
% 2.	Rise works better on cricket X dataset even with Time-series length is longer this is because in cricket X implicitly zero replacement works. If the dataset doesn’t have a zero replacement assumption then Rise will not perform better. 
% 3.	MSE also works better for cricket X dataset due to the same implicit zero replacement assumption.
% 4.	In the Earthquake dataset, we treat each time step as independent(which matches the SHAP assumption), and a sequence of time steps are used to classify the results instead of a single time step. This sequence of time step also matches with the SHAP assumption when it does permutation across different features ( or time step). SHAP doesn’t considers each time step 100 percentage, unlike NTE. In NTE we can consider a partial percentage of a time step.  Example. In the blip V3 dataset which had 111 000110, RNN found some boundary when we flipped one of the time steps with 0.55 value (even with each time step should have been treated as Boolean and not float value) but the model thinks it as float… The model finds the boundary value and our replacement strategy also follows similar principle.
% 5. CM VS NTE: Both of them uses TV norm to capture the sequence of time series but CM doesn’t take into the picture the time-series nature of data sets, while NTE uses a replacement strategy which is specific to the dataset.
% 6.	RISE does 100’s of random perturbation but for each perturbation, it uses 100 percentage of each timestep, it doesn’t consider part of the time step like 50 percentage of time step 1 or 60 percentage of time step 2, Instead after running 100’s of perturbations it says how many percentage times time step 1 is used and then gives weightage to that time step1. Say if time step 1 is used 20 times out of 100 runs then time step 1 gets 20 percentage weightage for good accuracy.
% 7.	SHAP is a superset of RISE algorithm but considers 100 percentage of permutations and for each time step, it uses 100 percentage of each time step like in RISE.
% 8.	NTE uses each time step partially, say for time step 1 it might say 0.3 percentage of time step 1 is needed for DNN to classify and it doesn’t need 100 percentage of time step 1. This is the basic difference between shap, rise and nte. The black box model also works similarly. i.e we work on Y-AXIS for each time step and take partial value of it but SHAP and RISE work on X-AXIS and considers N number of time steps but for each time step it takes 100 percentage of value.






















% RISE and MSE:

% 1. Wafer and Gun Point having 150 timesteps helps the case of RISE
% 2. Cricket X Dataset -> Zero replacement works, even with 500 timesteps, Rise and MSE performs better.
% 3. In Computers having a length of 720, RISE fails to perform

% RISE, Shap and MSE:
% 1. In Earthquakes, zero is a valid replacement and hence RISE, SHAP and MSE performs best
% 1.1 In 
% 2. SHAP performs the best because, the prediction is only dependent on X-axis and does not consider the magnitude of Y Axis, rather considers only the presence.

% What do we do?
% 1. We work on fine-grained (percentage replacement) control of replacement of each timestep instead of coarse grained (binary replacement) (RISE, SHAP and LIME)
% 2. If the magnitude of Y axis is not significance, NTE is an overkill for the given problem.
% 3. Even then we are close to the state-of-the art technique.

% }
